What do we know about Hugging Face? A systematic literature review and quantitative validation of qualitative claims

Background: Collaborative Software Package Registries (SPRs) are an integral part of the software supply chain. Much engineering work synthesizes SPR package into applications. Prior research has examined SPRs for traditional software, such as NPM (JavaScript) and PyPI (Python). Pre-Trained Model (PTM) Registries are an emerging class of SPR of increasing importance, because they support the deep learning supply chain. Aims: Recent empirical research has examined PTM registries in ways such as vulnerabilities, reuse processes, and evolution. However, no existing research synthesizes them to provide a systematic understanding of the current knowledge. Some of the existing research includes qualitative claims lacking quantitative analysis. Our research fills these gaps by providing a knowledge synthesis and quantitative analyses. Methods: We first conduct a systematic literature review (SLR). We then observe that some of the claims are qualitative. We identify quantifiable metrics associated with those claims, and measure in order to substantiate these claims. Results: From our SLR, we identify 12 claims about PTM reuse on the HuggingFace platform, 4 of which lack quantitative validation. We successfully test 3 of these claims through a quantitative analysis, and directly compare one with traditional software. Our findings corroborate qualitative claims with quantitative measurements. Our findings are: (1) PTMs have a much higher turnover rate than traditional software, indicating a dynamic and rapidly evolving reuse environment within the PTM ecosystem; and (2) There is a strong correlation between documentation quality and PTM popularity. Conclusions: We confirm qualitative research claims with concrete metrics, supporting prior qualitative and case study research. Our measures show further dynamics of PTM reuse, inspiring research infrastructure and new measures.

==> old/jason-notes.tex <==
So really there's a couple takeaways here.
The first thing is that there are claims that have been made about hugging face as a platform for pre-train model reuse that are motivating claims that people sort of have conducted kind of mini literature review that show up in their introductions, but they don't really substantiate those claims with actual measurements of population.
They simply have these claims as motivating reasons for their work.
An analysis and substantiation of these motivating claims through some form of qualitative or quantitative study would increase our understanding of PTM reuse as well as provide greater basis and motivation for these works.
It would also increase the validity of these works as they would have a more grounded basis.

Of the claims that we did have either quantitative or qualitative basis for, we selected a subset of those claims to measure actual quantitative measure measurement.
However, all of these claims would benefit from again a follow up measurement of some kind to ensure that these had not changed, as hugging face has grown exponentially from the time that these claims were last made.
Prior work in traditional software has shown that over time the patterns of contribution and reuse do tend to change in traditional software package registries, the analog that we compare against.
As a result, it is important to have a examination of the current trends and patterns of reuse to see if these are changing overtime or these are holding.

Something that was notable about all of these claims, was that few of them made comparisons to traditional software, and of the ones that did make comparisons, none of them made a contemporary quantitative measurement.
All of them that made comparisons comparisons on prior traditional software.
This is important for two reasons.
First, it is important to compare to traditional software as traditional software has had the time needed to show what the lifecycle and growth of a software package registry as well as what the maturation of software reuse processes looks like.
As a result, understanding the correlation, the strength of correlation between traditional software and train models would allow us to have a better sense of what the future might have important applications for researchers and users and policy makers on platforms.
The second reason why this is important is because even those comparisons that were made were not made quantitatively, which means that we don't have a real strong sense of what the current state of reuse is.
What I mean is that we don't have a sense of where in maturation process hugging faces because we don't have a actual quantitive comparison that says yes this is exactly the same as MPM or is right now, or is exactly the same as MPM or Pipi was five years ago ago.

Takeaways from this work is that there are tools that have been applied on small scales to further the understanding of pre-train model information but this has yet to be applied in a large scale to really give us a great data set to work with.
PeaTMOSS has its strengths but also has its flaws.
It's a good stepping stone for getting a great data set to compare to find information on hugging face, there are better next steps to take.
Something that again shows up when it comes to data set is whether they are up to date or not.
Again, hugging face has grown exponentially, even when compared to six months ago.
As a result, even snapshots that are several months old struggled to capture the current state of hugging face, which is a big deal because hugging face might be undergoing serious transformations that we are lagging behind in measuring because the tools that we have don't keep up-to-date.
As a result, having tools that keep up-to-date and up-to-date, understanding of the landscape is really really important for accurate measurements and understandings of the current state of reuse.


==> old/old.tex <==

\pagebreak 
\newpage


% GKT - Turned off centering, which was causing all content to be centered (jarring).

{\textbf{==========OLD CONTENT==========}}

\section{Background and Related Work}
This section covers Characterizing Software Package Registries, the Pre-Trained Model Supply Chain, and HuggingFace.
\section{Deep Neural Networks}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{archived/dnn.png}
    \caption{
    An example DNN, obtained from Wikipedia.
    \GKT{I'm not sure we need a picture of a DNN in the paper. We're mainly talking abotu PTMs and people can find DNN pictures just about anywhere.}
    \JD{Agree, please cut. An illustration of a PTM would be more useful.}
    }
    \label{fig:dnn-example}
\end{figure}

Deep Neural Networks (DNNs)
% (See Figure \ref{fig:dnn-example} \footnote{\url{https://vitalflux.com/deep-learning-neural-network-explained-simply-layman-terms/}})
have become popular in recent years as a solution to several novel problem domains (Computer Vision, Natural Language Processing, Audio Processing, etc.).
The advent of deep learning has precipitated a fundamental shift in computational methodologies, transitioning from the deterministic algorithms characteristic of traditional software to increasingly probabilistic and data-driven paradigms\cite{karpathy_software_2017}.
Deep learning typically operates through neural networks capable of assimilating datasets, thereby enabling them to make predictions or perform complex tasks\cite{lecun_deep_2015}. 
A variety of tools (PyTorch, ONNX, TensorFlow) have been developed to help engineers construct their own models from scratch.
However, the expertise, capital, time, and amount of data required to train a large DNN from scratch on a specific task is immense and discourages many from being able to create their own.
An alternative to creating DNNs from scratch is taking a checkpoint from a DNN that has already been trained, and reusing it in a variety of ways that range from direct reuse, to fine-tuning, to transfer learning, or optimization for size and efficiency \cite{jiang_peatmoss_2024}.
DNNs that are used in this way are known as Pre-Trained Models (PTMs).



\section{Pre-Trained Models}\label{sec:background-PTM}
This section covers PTMs 
% (\cref{sec:background-PTM})
and their reuse.
% (\cref{sec:background-PTMSupplyChain}).
  % and

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{archived/dnn-ptm.png}
    \caption[DNN reuse]{
    Figure 2 from \cite{jiang_empirical_2022} illustrating how a DNN may be reused as a PTM}
    \label{fig:enter-label}
\end{figure}

% A PTM represents a deep neural network that has been previously trained on a dataset, allowing it to make inferences or be repurposed for various downstream tasks.
A PTM embodies a DNN architecture that has undergone prior training with a specific dataset, incorporating a defined data pipeline, training regime, and learned parameters (``weights'').
This pre-training equips the PTM to perform inference or to be adapted for downstream applications\cite{davis2023JVA}.

Existing research has explored various methods for reusing deep learning models, such as feature extraction, transfer learning, data generation, and model compression\cite{Han2021PTM, Jiang2022PTMSupplyChain}.
For instance, DNNs can be pre-trained using large-scale unlabeled molecular databases and then fine-tuned over
specific chemical downstream tasks like molecular property prediction\cite{xia2023systematicSurveyofChemicalPTM}.
Additionally, models can be employed to annotate data or to synthesize new datasets through generative approaches\cite{Dube2019DataLabeling4TransferLearning, antoniou2017dataAugGenerativeAdvNetworks}.
Transfer learning enables models trained on generic datasets to refine their understanding of more detailed, downstream tasks, often resulting in enhanced performance on specialized datasets\cite{transferlearning}.
Furthermore, models can be optimized for size and efficiency to run on edge devices, a process known as model compression\cite{Deng2020ModelCompressionandHWAccelerationforNN}. 
Thanks to this range of reuse modes, in recent years PTMs have become increasingly popular\cite{kathikar2023assessingHFVulnerabilities, castano2023exploring}, with the total number of open-source PTM packages seeing a consistent increase on a monthly basis\cite{castano2023exploring}.

\subsection{Software Supply Chains}
Software does not exist in a vacuum.
There exists a software supply chain that connects software component creators to reusers \cite{dey_are_2018, boyens_case_2020, boyens_cybersecurity_2022, boyens_key_2021}. 
The components of the supply chains that we are interested in are:
\begin{table}[h]
    \centering
    \caption[Software Supply Chain Actors and Components]{Software Supply Chain Actors and Components\cite{boyens_cybersecurity_2022, ladisa_sok_2023}.}
    \begin{tabular}{p{0.24\columnwidth} p{0.7\columnwidth}}
    \toprule
     \textbf{Component}       & \textbf{Description} \\ 
     \midrule
    1. Packages        & The actual software that can be reused \\ 
    2. Contributors    & Engineers who produce and maintain Packages \\ 
    3. Reusers         & The downstream reusers of Packages \\ 
    4. Systems         & End-result systems that use Packages \\
    5. Registries      & Platforms that host Packages for reuse \\ 
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

The supply chain generally works as follows: Software Component Contributors (2) create Software Packages (1) that accomplish specific tasks.
These components are uploaded to a Software Package Registry (5) that stores these packages and allows for future reuse.
Other software engineers looking to replicate functionality in a short period of time will participate in the ecosystem as a reuser (3) who selects uploaded software components from a registry and incporates them into their own code to create a software system (4).
This software system can be an end-user facing application, or can be another package that is uploaded to a registry for reuse.

\subsection{Software Package Registries}
Software registries are a key component of the software supply chain that provides a platform for engineers to share their work.
These registries often provide package metadata, social features, and tools that enable version management and streamline package selection, downloading, and assembly.
These result in an ecosystem that is rich in information about components and users.
NPM (JavaScript) and \pypi (Python) are particularly studied software registries, due to the popularity of the associated programming languages~\cite{zerouali_formal_2019, pinckney_large_2023, wittern_look_2016, zerouali_empirical_2018, bommarito_empirical_2019, guo_empirical_2023, gu_investigating_2023, zerouali_diversity_2019, zimmermann_small_nodate, stringer_technical_2020, zahan_what_2022, decan_empirical_2019}.
HuggingFace is an emerging PTM registry, with similarly high adoption.
A greater explanation of HuggingFace is present in \cref{ch:PTM Supply Chain ESEM} and \cref{ch:HuggingFace ESEM}.
% \cref{fig:PackagePopularity} provides a quantitative demonstration of the extensive adoption and rising popularity of PTMs on HuggingFace. 
% Previous research indicates that the popularity and adoption rate of Hugging Face's models are comparable to those of other established software package registries, including npm and PyPI\cite{Jiang2022PTMReuse}.

% \begin{table}[h]
% \centering
% %\small
% \caption[Comparison of package counts and download figures for the top 10\% of PTMs on HuggingFace.]{
%   Comparison of package counts and download figures for the top 10\% of PTMs on HuggingFace.
%   Data for August 2022 is sourced from the PTMTorrent dataset\cite{jiang2023ptmtorrent}.
%   The August 2023 data is obtained from our dataset.
%   This comparison highlights the growth of PTM usage over a one-year period (\ie doubling).
%   }
% \label{tab:popularity-comparison}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Hugging Face Statistics} & \textbf{Aug. 2022} & \textbf{Aug. 2023} \\
% \midrule
% \# packages of all PTMs & 124\ K  & 282\ K \\
% %\midrule
% % \# packages of all PTMs & \NUMPTMTorrentHFPTMs  & \NEWnumberOfPTMs \\
% % \# downloads of top 10\% PTMs & 268,961,151 & 587,031,839 \\
% \# downloads of top 10\% PTMs & 269 billion & 587 billion \\
% \bottomrule
% \label{fig:PackagePopularity}
% \end{tabular}
% \end{table}


\subsection{Characterizing Software Registries}
A significant number of registries across a wide range of languages and software types have sprung up over the years \cite{decan_empirical_2019, }.
Understanding these registries begins at first with understanding the inter-connectedness of the padckages, resuling in a dependency graph often being created as an artifact
\cite{zerouali_empirical_2018, zimmermann_small_nodate,
decan_evolution_2018,
ahmed_case_2017,
abate_dependency_2012,
blanthorn_evolution_2019,
zhang_how_2020,
gu_investigating_2023,
zerouali_diversity_2019,
dey_patterns_2019,
kula_visualizing_2014}.
This dependency graph is then used to characterize the preferences in contributions of contributors \cite{dey_patterns_2019, zhang_how_2020, ahmed_case_2017}, the way that users responded to updates to a package \cite{pinckney_large_2023,
zerouali_empirical_2018,
wan_are_2021,
hora_how_2018,
decan_evolution_2018,
stringer_technical_2020}, as well as information about the popularity of packages \cite{wittern_look_2016,zerouali_diversity_2019}.
The insights from these studies and more has contributed to further studies on the security implications and risks of the ecosystems \cite{boyens_case_2020, zimmermann_small_nodate,
boyens_cybersecurity_2022,
boyens_key_2021,
zahan_what_2022}.
The body of work generated by these studies was influential in informing best practices in security and ecosystem policies
% \TODO{[justification]}
, as well as informing the reuse process for general engineer.
% \TODO{[justification]}.

% \TODO{Subsection about deep learning, datasets, etc. Check MSR paper for a possible figure to imitate}
\subsection{The Pre-Trained Model Software Supply Chain} \label{ch:PTM Supply Chain ESEM}

Deep Neural Networks (DNNs) have become popular in recent years as a solution to several novel problem domains (Computer Vision, Natural language processing, Audio Processing).
A variety of tools (PyTorch, ONNX, TensorFlow) have been developed to help engineers construct their own models from scratch.
However, the expertise, capital, time, and amount of data required to train a large DNN from scratch on a specific task is immense and disqualifies many from being able to create their own.
An alternative to creating DNNs from scratch is taking a checkpoint from a DNN that has already been trained, and reusing it in a variety of ways that range from direct reuse, to fine-tuning, to transfer learning, or optimization for size and efficiency \cite{jiang_peatmoss_2024}.
DNNs that are used in this way are known as Pre-Trained Models (PTMs).

Using PTMs allows for users to capture much of the functionality of creating a DNN from scratch without the significant investment of time and capital.
As a result, the usage of PTMs has risen \cite{jiang_empirical_2022, kathikar_assessing_2023}.
In order to facilitate this reuse, a number of registries specialized in PTMs, referred to as Model Zoos, have come into existence.
There are a variety of model zoos that exist.
They fall into 1 of 3 types: Open, Gated, and Commercial \cite{jiang_empirical_2023}.
Of these three types, Open model zoos most resembles popular traditional software registries, as they allow for free contribution.
The most popular open model zoo that is HuggingFace, which is the focus of this paper.

\subsection{Hugging Face}\label{ch:HuggingFace ESEM}
The largest and most popular platform for PTM reuse is the Open Model Zoo HuggingFace, which currently hosts more than 591k models.
HuggingFace operates similarly to other software registries; it contains metadata about PTMs, social features to connect users, and version management.
Also like other registries, it provides a cli to facilitate reuse, as well as a variety of tools to enable reuse.
However, given the nature of PTMs, it is sometimes difficult for potential reusers to store and run a complete PTM on their machine.
As a result, HuggingFace also provides APIs to allow for access to PTMs without incorporating the model itself into the development/runtime environment.

Previous work has examined the role of HuggingFace as a platform for hosting and storing PTMs, similar to GitHub for traditional software repositories \cite{taraghi_deep_2024}.
Previous work has also examined the ways in which HuggingFace has begun to facilitate PTM reuse \cite{nahar_dataset_2023, taraghi_deep_2024}.
What they found is that HuggingFace, along with all PTM registries, show the a pattern of reuse that implies PTM selection is much more important than PTM synthesis.
This is consistent with the body of work present on package selection.
Researcher have contributed methods and tools for users to evaluate PTMs to identify the ideal models for their downstream projects \cite{you_logme_2021, talmor_olmpics-what_2020, bassignana_evidence_2022, chen_how_2023, shao_not_2022, chiang_transferability_2022}.
These evaluation tools benchmark PTM performance for inter-model comparison, allowing for downstream reusers to select the PTM that best fits their needs.
As a result, prior work indicates that PTM selection is more vital than PTM synthesis.

% \TODO{[cite more]}.
Prior work has also examined the methods by which HuggingFace facilitates the reuse of the models it hosts, as well as analyzed the security implications these new methods have on the resulting software supply chain \cite{jiang_empirical_2022, jiang_empirical_2023}.
However, we have not found a work that provides an empirical comparison between the patterns of reuse that HuggingFace facilitates and that of traditional software registries.

% \subsection{PeaTMOSS}
% PeaTMOSS is a dataset that captures the metadata of 281,638 Pre-Trained Models hosted on HuggingFace and PyTorch, and connects them to 28,575 GitHub repositories that reuse PTMs, creating 44,337 mappings from 15,129 downstream GitHub repositories to 2,530 PTMs. \cite{jiang_peatmoss_2024}.
% PeaTMOSS also contains 59,011 Discussions from HuggingFace, as well as 827,856 Pull Requests and 631,007 Issues from GitHub. \cite{jiang_peatmoss_2024}
% PeaTMOSS was originally created to facilitate work examining PTM packages across multiple model zoos \cite{jiang_ptmtorrent_2023}.
% The rapid emergence and dominance of HuggingFace and PyTorch as platforms for PTM reuse, as well as the richness of metadata on the HuggingFace platform compared to all other platforms resulted in a reduction of scope to focus entirely on HuggingFace and PyTorch \cite{jiang_peatmoss_2023}.
% The original Model Zoo metadata was eventually augmented with downstream GitHub repositories that reused PTMs from either HuggingFace or PyTorch, in order to create a dataset that contained information about both model contributors and users \cite{jiang_peatmoss_2023}.
% Artifacts related to model contribution (HuggingFace discussions) and downstream reuse (GitHub Issues and Pull Requests) were also captured in the dataset \cite{jiang_peatmoss_2023}.
% The HuggingFace metadata was later augmented using a Large Language Model to further extract details from the relatively unstructured metadata format of HuggingFace model cards \cite{jiang_peatmoss_2024}.
% The significant amount and quality of data available in PeaTMOSS allows for the calculation of metrics originally used to measure traditional software registries.

\subsection{Summary and Knowledge Gaps}
Software Supply Chains describe the connections between creators, packages, and users.
Software registries are collaborative platforms that unite contributors, users, and packages, and streamline package management processes.
The introduction of PTMs to the Software Supply Chain is only beginning to be examined.

PTMs have novel applications and attributes compared to traditional software.
Prior work has established that software engineers claim that the problem of PTM reuse is selection over synthesis, with efforts in this field seeming to confirm this claim.
However, we have yet to verify these claims with quantitative data.
% \JD{Perhaps this paragraph should just end here.}
% For example, we do not yet know how centralized contribution to the PTM Supply Chain is, nor how interconnected PTMs are, nor how stable \JD{what does `stable' mean?} PTM usage is.
% We lack quantified evidence to compare to the qualitative data from prior work.
% \JD{Perhaps this paragraph should just end here.}
% For example, we do not yet know how centralized contribution to the PTM Supply Chain is, nor how interconnected PTMs are, nor how stable \JD{what does `stable' mean?} PTM usage is.
% We lack quantified evidence to compare to the qualitative data from prior work.

% \section{Research Questions} \label{Research Questions}
% % The purpose of this paper is to compare the ways engineers interact with the HuggingFace ecosystem \JD{Well, we want to know about PTMs (engineering practice) and we specifically look at HF (context in which to study that practice). It is important to draw this distinction because it helps the reader understand why we made the choices we did and how specific to HF our results are} compared to traditional registries.

% % \JD{There is no statement of RQs. What are your RQs?}

% Research Questions are designed to examine the registries from several perspectives:
% \begin{enumerate}
%     \item What are the Package-to-Package relationships?
%     \item What are the Package-to-Reuser relationships?
%     \item What are the Contributor-to-Package relationships?
%     \item What are the Reuser-to-Package relationships?
% \end{enumerate}
% % \begin{enumerate}
% %     \item A contributor to the registry looking downstream at packages and eventual reusers
% %     \item A reuser of the registry looking upstream at packages selected and the creators
% %     \item Packages looking outward at other packages, the maintainers that create them, and the reusers that use them
% % \end{enumerate}

% % Research Questions:
% % \JD{These questions are asking bigger questions than you are answering. Maybe simplify the questions, to just ``Are they the same along dimension X?'' That is what you actually answer, right?}
% % \begin{enumerate}
% %     \item How do package relationships with each other change across traditional software and PTM registries?
% %     \item How do package reuse permissions affect their usage across traditional software and PTM registries?
% %     \item How does the reach of contributors compare across traditional software and PTM registries?
% %     \item How does the selection of packages compare across traditional sofware and PTM registries?
% % \end{enumerate}



% Each of these research questions will be answered by several metrics that evaluate the category on an axis
% \subsection{Package-to-Package}
% Package-to-Package Relationships examine how packages are utilized by other packages.
% \subsubsection{Dependency Trees}
% Dependecy Trees are an important way to measure the reach packages have within an ecosystem.
% This reach is important in understanding how updates to the package, and vulnerabilites that the package has can impact other packages, and the ecosystem as a whole.
% As a result, understanding the reach of various models is important in the context of PTMs.
% PTMs also have the added dimension of architectures, where architectures can have a reach beyond just a single model.
% As a result, building a graph that examines the reach of both models and architectures is important.
% This graph also facilitates questions about user collaboration and Industry Sponsorship.

% \subsection{Package-to-Reuser}
% Package-to-Reuser examines how Packages are selected by downstream software projects, as well as how the packages are meant to be reused.
% \subsubsection{Dependent Repositories}
% Dependent Repositories refers to downstream projects that utilize a package.
% This is a subset of a dependency, in that a package is still being required by a software project.
% However, these projects are often aimed either at non-software engineer end-users, or to implement functoinality that is not worth integration into other packages \needcite{}.
% % However, the including project is not intended to be reused by other packages, and is often more likely to be meant for use by the general public in a non-developmental capacity, rather than a package which is often meant for software engineers so that they can create new packages as well as general public intended software.
% % This has two important implications.
% % (1) There will not be an indirect series of dependencies that arises through the inclusion of this package into another and (2) since the including repository does not plan to be included in another project, it is more likely to have an end product and have different considerations.

% \subsubsection{Licenses}
% Software licenses are important to understand how the creator of a software component intended for it to be reused.
% Software licenses generally fall into one of several categories, and can range from completely open source, to completely proprietary.
% Their study can reveal patterns of contribution and opinions on the openness and reusability of the software on a platform.
% This is particular interesting when it comes to HuggingFace, as it is possible that the differing nature of the models themselves, as well as the variety of increased moral and ethical concerns around the software itself would lead to a openness of software on many models.
% It is also compelling to examine how different licenses and the permissions that they grant impact the reuse and popularity of the license software.

% \subsection{Contributor-to-Package}
% Contributor-to-Package examines how Contributors influence Packages.
% \subsubsection{User Reach}
% User Reach refers to the influence that package contributors have on downstream packages and reusers.
% % This has important implications for security, as revealing the impact power users have helps revealw their impact should they become a bad actor.
% % It is also reveals how healthy an ecosystem is in terms of its bus factor.
% % This holds significant implications for security, as understanding the influence of power users illuminates the potential risks should they turn into malicious actors.
% Because of the interconnectedness of modern software package registries, the reach of a user extends beyond the packages that they directly contribute to, and includes downstream dependent packages and projects.
% As a result, working from a dependency graph is incredibly important to fully understand user reach.
% Understanding the influence of power users in particular illuminates potential risks should they turn into malicious actors and sheds light on the health of an ecosystem by revealing its resilience in terms of the bus factor.
% % User Reach reach is also something that built off of dependencies, as a users reach isn't just measured in the amount of projects that they actively contribute to.


% \subsection{Reuser-to-Package}
% This examines how people make use of the registry with an upstream view.

% \subsubsection{Popularity}
% The selection of software components is an important part of characterizing a software registry.
% In particular, evaluating the turnover at the top of the most popular packages on a software registry can help inform the nature of the packages on the platform itself.
% A registry has high turnover or low, that can indicate the stability of top packages on a platform, as well as characterize, whether or not new packages are of likely importance to all packages.
% This thing that is helpful as well because it also reveals a little bit whether it is more important to contribute to pre-existing packages or to just add new packages from scratch.

% % \subsubsection{Version Management}
% % Version Management looks at how downstream users of PTMs manage updates to a PTM package.
% % This is evaluated based on the Technical Lag that exists.
% % In traditional software, Technical Lag is a measure of how long it takes for downstream software packages to update to the latest version of a dependency once an update is made.
% % Though there are issues with this metric (every update can include bugs, new vulnerabilites, and bloat that may not make sense for a downstream package to take on) in the realm of PTMs these concerns are lessened.
% % In general, given the nature of PTMs, it is more likely for a downstream user to always want to use the most recent version of a PTM.
% % As a result, the measure of Techncial Lag is important.


% \begin{table*}[h]
% \caption{License Category Definitions and Examples}
% \label{tab:licenses}
% \begin{tabular}{p{0.15\textwidth}p{0.65\textwidth}p{0.2\textwidth}}
% \toprule
% \textbf{License} \textbf{Category} & \textbf{Description} & \textbf{Examples} \\
% \midrule
% Permissive & This type of license does not require changes to existing code to be published under the same license as long as they include a copy of the license and attribution to the original authors in the copies or derivative works. & Apache License, BSD License, MIT License, Artistic License 2.0 \\ \hline
% Weak Copyleft & This type allows users to change the source code into proprietary application/software, as long as the source code is made available under the same license. Code using the existing code does not have to be published under the same license. & Mozilla Public License (MPL), Lesser GNU Public License (LGPL), Eclipse Public License (EPL) \\ \hline
% Strong Copyleft & This is the most restrictive type. Code using the existing code must be published under the same license. & GNU General Public License (GPL), GNU Affero General Public License (AGPL) \\ \hline
% Public & This type is the least restrictive type. Use of the material is made free from restrictions from copyright or database laws, so that others may freely build upon the work, to the full extent possible. "No Rights Reserved". & CC0 Public Domain License \href{https://creativecommons.org/public-domain/cc0/}{(Link)} \\ \hline
% No License & Without a license, in the case of software typically adherent to the default rules stated by the terms of service if code is located in an hosting platform such as GitHub or Hugging Face. &  \\ \hline
% Other & None of the above, these licenses are not the focus of this study, and are not a significant part of our dataset. &  \\ 
% \bottomrule
% \end{tabular}
% \end{table*}
\section{Research Questions} \label{Research Questions}
% The purpose of this paper is to compare the ways engineers interact with the HuggingFace ecosystem \JD{Well, we want to know about PTMs (engineering practice) and we specifically look at HF (context in which to study that practice). It is important to draw this distinction because it helps the reader understand why we made the choices we did and how specific to HF our results are} compared to traditional registries.

% In order to characterize each registry, we examined two themes:

% \noindent{\textbf{Theme 1: Package Contribution}}
% \begin{itemize}
%     \item[\textbf{RQ1:}] How do \ctp relationships differ between traditional software and PTM registries?
% \end{itemize}
% \noindent{\textbf{Theme 2: Package Evolution}}
% \begin{itemize}
%     \item[\textbf{RQ2:}] How do \ptp relationships differ between traditional software and PTM registries?
% \end{itemize}
% \noindent{\textbf{Theme 3: Package Reuse}}
% \begin{itemize}
%     \item[\textbf{RQ3:}] How do \ptr relationships differ between traditional software and PTM registries?
%     \item[\textbf{RQ4:}] How do \rtp relationships differ between traditional software and PTM registries?
% \end{itemize}

% \JD{There is no statement of RQs. What are your RQs?}
To restate: the hy  pothesis I test is \textit{\hypothesis}.

In order to test this hypothesis, I quantitatively characterize Package Registries on two dimensions:
(1) \textit{Package Evolution}, and
(2) \textit{Package Reuse}

\noindent{\textbf{Research Question 1: Package Evolution}}\\
Package evolution describes the way that packages on a given software registry depend each other to improve their functionality.
Prior work has examined this through the lens of the evolution of dependency network network on platforms \cite{decan_evolution_2018, wittern_look_2016}.
This has given insight into how packages take on functionality from other packages to provide new functionality, which has made the interconnectedness of packages on the registry more well-known.
Measuring this aspect is crucial because it helps clarify the overall dynamics of software development.
In traditional software development, there is pre-existing functionality that developers prefer not to build from scratch.
Instead, they rely on existing packages that offer these basic functionalities.
Developers then integrate these packages into their own projects, extending them with specialized, niche functionalities to enhance and tailor their software to specific needs.
This process underscores the importance of understanding how software components are reused and extended across different applications.
% This is an important thing to measure as this reveals in general like what the hell is going on right because we don't really have an understanding well traditional software what happens is that people that you know things software? What happens is you have a wide amount of basic functionality that you don't wanna have to implant yourself and so in order to provide that basic functionality with specialized niche, additional functionality, what you do is you look to other packages to provide that and include that in your package and then you provide and extend your own spe functionality.

\noindent{\textbf{Research Question 2: Package Reuse}}\\
Package reuse in non-engineer focused software projects specifically examines how downstream users leverage existing packages.
Typically, engineers combine multiple packages to achieve desired functionalities.
Historically, research has focused on downstream project dependency amounts to determine the extent of software package usage.
This has also been explored from the perspective of package inclusion in projects, identifying which packages are most widely used across a platform.
The concept of permanency in usage relates to the frequency of turnover among the most popular packages \cite{wittern_look_2016}.
In traditional software ecosystems, there's a tendency for popular packages to perpetuate their use --- a ``rich get richer'' scenario --- because the cost of replicating their functionality is often higher than simply continuing to use them.
Identifying a deviation from this pattern in the pre-trained model domain would be noteworthy.
% Package reuse looks downstream specifically at how people reuse packages in non-engineer focused software projects.
% Similarly to packages, generally engineers synthesize several packages together in order to obtain functionally.
% In prior software, this has looked at similarly dependencies to see how many software packages are being used
% This is also been examined from the point of view of packages being included in project to see which packages are the most widely used
% This includes both what is the most widely used in general as unlike fundament how centralized is use on a platform as well as permanent uses.
% Permanency of us refers to the turnover of the most popular packages.
% In traditional software, we have a kind of rich get richer situation where once a package is established as a popular package, it is continued to be used downstream by other applications as the cost to replicate that functionality is not worth simply just using that functionality.
% As a result, if this were to be different in the pre-model domain that would be significant.

% \begin{enumerate}
%     \item A contributor to the registry looking downstream at packages and eventual reusers
%     \item A reuser of the registry looking upstream at packages selected and the creators
%     \item Packages looking outward at other packages, the maintainers that create them, and the reusers that use them
% \end{enumerate}

% Research Questions:
% \JD{These questions are asking bigger questions than you are answering. Maybe simplify the questions, to just ``Are they the same along dimension X?'' That is what you actually answer, right?}
% \begin{enumerate}
%     \item How do package relationships with each other change across traditional software and PTM registries?
%     \item How do package reuse permissions affect their usage across traditional software and PTM registries?
%     \item How does the reach of contributors compare across traditional software and PTM registries?
%     \item How does the selection of packages compare across traditional sofware and PTM registries?
% \end{enumerate}



% Each of these research questions will be answered by several metrics that evaluate the category on an axis
% \subsection{Package Contribution}
% Hello
% \subsubsection{\ctp}
% Contributor-to-Package examines how Contributors influence Packages.

% \ul{User Reach}
% User Reach refers to the influence that package contributors have on downstream packages and reusers.
% % This has important implications for security, as revealing the impact power users have helps revealw their impact should they become a bad actor.
% % It is also reveals how healthy an ecosystem is in terms of its bus factor.
% % This holds significant implications for security, as understanding the influence of power users illuminates the potential risks should they turn into malicious actors.
% Because of the interconnectedness of modern software package registries, the reach of a user extends beyond the packages that they directly contribute to, and includes downstream dependent packages and projects.
% As a result, working from a dependency graph is incredibly important to fully understand user reach.
% Understanding the influence of power users in particular illuminates potential risks should they turn into malicious actors and sheds light on the health of an ecosystem by revealing its resilience in terms of the bus factor.
% % User Reach reach is also something that built off of dependencies, as a users reach isn't just measured in the amount of projects that they actively contribute to.

\subsection{Package Evolution}
% \subsubsection{\ptp}
% Package-to-Package Relationships examine how packages are utilized by other packages.

\ul{Dependent Packages:}
Dependent Packages are an important way to measure the reach packages have within an ecosystem.
This reach is important in understanding how updates to the package, and vulnerabilites that the package has can impact other packages, and the ecosystem as a whole.
As a result, understanding the reach of various models is important in the context of PTMs.
PTMs also have the added dimension of architectures, where architectures can have a reach beyond just a single model.
As a result, building a graph that examines the reach of both models and architectures is important.
This graph also facilitates questions about user collaboration and Industry Sponsorship.

\ul{Package Dependencies:}
Package dependencies is a good way to look at the inverse of dependent packages.
This looks upstream from the point of view of a package that is using other packages for functionality and indicates how much functionality is inherited from a number of sources versus from a single specific source.
This uses the same graph as dependent packages just looking in the opposite direction rather than looking at packages that include a package. It looks from the point of view over package and looks at what packages are included by that package.


\subsection{Package Reuse}
% \subsubsection{\ptr}
% Package-to-Reuser examines how Packages are selected by downstream software projects, as well as how the packages are meant to be reused.

\ul{Dependent Repositories:}
Dependent Repositories refers to downstream projects that utilize a package.
This is a subset of a dependency, in that a package is still being required by a software project.
However, these projects are often aimed either at non-software engineer end-users, or to implement functoinality that is not worth integration into other packages.
% \TODO{[]}.
% However, the including project is not intended to be reused by other packages, and is often more likely to be meant for use by the general public in a non-developmental capacity, rather than a package which is often meant for software engineers so that they can create new packages as well as general public intended software.
% This has two important implications.
% (1) There will not be an indirect series of dependencies that arises through the inclusion of this package into another and (2) since the including repository does not plan to be included in another project, it is more likely to have an end product and have different considerations.

% \ul{Licenses:}
% Software licenses are important to understand how the creator of a software component intended for it to be reused.
% Software licenses generally fall into one of several categories, and can range from completely open source, to completely proprietary.
% Their study can reveal patterns of contribution and opinions on the openness and reusability of the software on a platform.
% This is particular interesting when it comes to HuggingFace, as it is possible that the differing nature of the models themselves, as well as the variety of increased moral and ethical concerns around the software itself would lead to a openness of software on many models.
% It is also compelling to examine how different licenses and the permissions that they grant impact the reuse and popularity of the license software.

% \subsubsection{\rtp}
% This examines how people make use of the registry with an upstream view.

\ul{Popularity:}
The selection of software components is an important part of characterizing a software registry.
In particular, evaluating the turnover at the top of the most popular packages on a software registry can help inform the nature of the packages on the platform itself.
A registry has high turnover or low, that can indicate the stability of top packages on a platform, as well as characterize, whether or not new packages are of likely importance to all packages.
This has additional utility as it reveals whether it is more important to contribute to pre-existing packages or to just add new packages from scratch.

% \subsubsection{Version Management}
% Version Management looks at how downstream users of PTMs manage updates to a PTM package.
% This is evaluated based on the Technical Lag that exists.
% In traditional software, Technical Lag is a measure of how long it takes for downstream software packages to update to the latest version of a dependency once an update is made.
% Though there are issues with this metric (every update can include bugs, new vulnerabilites, and bloat that may not make sense for a downstream package to take on) in the realm of PTMs these concerns are lessened.
% In general, given the nature of PTMs, it is more likely for a downstream user to always want to use the most recent version of a PTM.
% As a result, the measure of Techncial Lag is important.


% \begin{table*}[h]
% \caption{License Category Definitions and Examples}
% \label{tab:licenses}
% \begin{tabular}{p{0.13\textwidth} p{0.57\textwidth} p{0.25\textwidth}}
% \toprule
% \textbf{License} \textbf{Category} & \textbf{Description} & \textbf{Examples} \\
% \midrule
% Permissive & This type of license does not require changes to existing code to be published under the same license as long as they include a copy of the license and attribution to the original authors in the copies or derivative works. & Apache License, BSD License, MIT License, Artistic License 2.0 \\ 
% \midrule
% Weak Copyleft & This type allows users to change the source code into proprietary application/software, as long as the source code is made available under the same license. Code using the existing code does not have to be published under the same license. & Mozilla Public License (MPL), Lesser GNU Public License (LGPL), Eclipse Public License (EPL) \\ 
% \midrule
% Strong Copyleft & This is the most restrictive type. Code using the existing code must be published under the same license. & GNU General Public License (GPL), GNU Affero General Public License (AGPL) \\ 
% \midrule
% Public & This type is the least restrictive type. Use of the material is made free from restrictions from copyright or database laws, so that others may freely build upon the work, to the full extent possible. &  "No Rights Reserved", CC0 Public Domain License  \\ % \href{https://creativecommons.org/public-domain/cc0/}{(Link)} 
% \midrule
% No License & Without a license, in the case of software typically adherent to the default rules stated by the terms of service if code is located in an hosting platform such as GitHub or Hugging Face. &  \\ 
% \midrule
% Other & None of the above, these licenses are not the focus of this study, and are not a significant part of our dataset. &  \\ 
% \bottomrule
% \end{tabular}
% \end{table*}

% \section{Methods}

% \JD{ESEM call states that: Papers must contain an explicit description of the empirical strategy used or investigated. See the website for more details about what they want to see.}

% % What follows are the methods used to generate data for comparison between traditional software registries (\npm and \pypi) and HuggingFace.

% % \JD{You must also explain the comparison itself. How will you decide whether PTM registry is similar or different from traditional? What threshold or measure will you use?}
% % \JD{Do you have a hypothesis? State it clearly.}
% We adopt a systematic framework to measure both the qualitative and quantitative attributes of traditional software registries (\npm and \pypi) and HuggingFace.
% To assess similarities or distinctions, we leveraged a comprehensive suite of metrics describing package interdependency networks, the extent of contributor influence, and patterns of reuse.
% These metrics serve to quantify critical aspects, facilitating a cross-registry comparison.
% The criteria for establishing similarity or divergence begins with an initial visual analysis, subsequently eventually corroborated through comparative analytical techniques, including t-tests, to ensure a robust, evidence-based evaluation.
% % To assess whether HuggingFace is similar to or distinct from traditional registries, we employed a set of metrics encompassing package interdependency networks, contributor influence, and reuse patterns.
% % These metrics quantified these key components to allow for comparison across registries.
% % The decision criteria for similarity or difference will be based on visual analysis that is eventually supported by comparative analysis techniques such as t-tests.
% % The decision criteria for similarity or difference will be based on statistical significance thresholds determined through comparative analysis techniques such as t-tests or effect size measurements, ensuring that observed differences are not merely by chance.

% We have a clear hypothesis: \textit{The contextual and technical distinctions between PTM packages and traditional software packages manifest in measurable differences in their interdependency networks, contributor impacts, and selection for downstream reuse.}
% We expect every metric to demonstrate an obvious difference between \hf and traditional software registries.
% % This hypothesis seeks to explore the extent to which the unique characteristics of PTMs—arising from their development, deployment, and use cases—translate into observable differences in registry dynamics when compared to traditional software ecosystems.
% % Our analysis aims to test this hypothesis through empirical data, offering insights into the implications of these differences for developers, users, and the broader software engineering community

% \subsection{Dataset}
% There exist several datasets that capture information about HuggingFace \needcite{}.
% After review of several datasets, we decided to use the PeaTMOSS deataset \cite{jiang_peatmoss_2024}.
% The model metadata, the model relationships, and downstream relationships with GitHub repositories captured within the dataset allowed us to compare HuggingFace to traditional software registries.
% % PeaTMOSS is a dataset that captures the metadata of 281,638 Pre-Trained Models hosted on HuggingFace and PyTorch, and connects them to 28,575 GitHub repositories that reuse PTMs, creating 44,337 mappings from 15,129 downstream GitHub repositories to 2,530 PTMs. \cite{jiang_peatmoss_2024}.
% % PeaTMOSS also contains 59,011 Discussions from HuggingFace, as well as 827,856 Pull Requests and 631,007 Issues from GitHub. \cite{jiang_peatmoss_2024}
% % PeaTMOSS was originally created to facilitate work examining PTM packages across multiple model zoos \cite{jiang_ptmtorrent_2023}.
% % The rapid emergence and dominance of HuggingFace and PyTorch as platforms for PTM reuse, as well as the richness of metadata on the HuggingFace platform compared to all other platforms resulted in a reduction of scope to focus entirely on HuggingFace and PyTorch \cite{jiang_peatmoss_2023}.
% % The original Model Zoo metadata was eventually augmented with downstream GitHub repositories that reused PTMs from either HuggingFace or PyTorch, in order to create a dataset that contained information about both model contributors and users \cite{jiang_peatmoss_2023}.
% % Artifacts related to model contribution (HuggingFace discussions) and downstream reuse (GitHub Issues and Pull Requests) were also captured in the dataset \cite{jiang_peatmoss_2023}.
% % The HuggingFace metadata was later augmented using a Large Language Model to further extract details from the relatively unstructured metadata format of HuggingFace model cards \cite{jiang_peatmoss_2024}.
% % The significant amount and quality of data available in PeaTMOSS allows for the calculation of metrics originally used to measure traditional software registries.


% \subsection{\ptp}
% \subsubsection{Dependencies}
% To measure \ptp relationships, dependencies were examined.
% In the context of PTMs, dependencies exist not as a persistent connection to another PTM, but as a checkpoint from which a model was taken from.
% However, the idea of a dependency tree remains the same.
% In the PeaTMOSS dataset, the table "model\_to\_base\_model" connects models to the original model that they diverged from.
% This table was created using the DARA pipeline, as mentioned in \cite{jiang_peatmoss_2024}.
% The graphs are generated as follows:
% The number of dependent packages ($D_p$) is the number of direct dependents ($N_d$) that a package has:
% \begin{equation}
% D_p = N_d
% \end{equation}

% The number of dependent packages for a PTM ($D_{ptm}$) is the number of models that use it as a checkpoint to train from ($M_c$):
% \begin{equation}
% D_{ptm} = M_c
% \end{equation}


% \subsection{\ptr}
% To measure \ptr relationships, dependent repositories and software licenses were examined.
% \subsubsection{Dependent Repositories}
% The number of dependent repos ($R_d$) is the number of repositories that directly include the package ($R_i$), whether it is traditional software or a PTM :
% \begin{equation}
% R_d = R_i
% \end{equation}

% \subsubsection{Licenses}
% Licenses are categorized as shown in \ref{tab:licenses}.
% The raw licenses for each platform are available in both the Packages and PeaTMOSS datasets.
% For each platform, the licenses from the top 10\% of packages were gathered, along with their frequency.
% The licenses were then consolidated based on the embeddings generated, in order to simplify classification.

% Licenses were approached this way because of the lack of standardization in reporting practices for software licenses.
% This resulted in a large amount and variety of raw license data.
% As an example, PyPi had 9,340 different licenses within its top 10\% of packages, with licenses such as
% Apache 2.0, Apache Software License, Apache License 2.0, Apache-2.0, "Apache License, Version 2.0", Apache, and Apache License Version 2.0 all being counted differently.
% Using this method, the number of unique licenses on PyPi was consolidated down to 400, which allowed for a more in-depth manual review of license classifications.

% While it has not been done specifically in the realm of license names, prior work has used embeddings compared pair-wise using cosine similarity to classify things \cite{mathur_putting_2019, zhang_bertscore_2019, kim_evaluating_2022, quan_efficient_2019}.
% After doing it this way and manually reviewing, I found that the consolidation was \TODO{XX\%} effective.

% This consolidation was done as follows:

% % \JD{It is unclear why you are doing it this way as opposed to a more formal/sound approach. Give some rationale for the use of LLMs and cosine embeddings. (What else did you consider? Why did you do it this way? Has anyone else done it this way? Why doesn't other people's approach work for you?)}

% Given a series of software licenses, for each license $L_i$, the process is as follows:

% \begin{enumerate}
%     \item Obtain the first up to 40 characters of each software license $L_i$:
%     \[ L_{i,40} = \text{first 40 characters of } L_i \]

%     \item Generate embeddings for each license excerpt $L_{i,40}$:
%     \[ E_i = E(L_{i,40}) \]
%     Where $E_i$ is the embedding for the $i^{th}$ license's excerpt.

%     \item Compute the cosine similarity between embeddings $E_i$ and $E_j$ for licenses $i$ and $j$:
%     \[ C(E_i, E_j) = \frac{E_i \cdot E_j}{\|E_i\|\|E_j\|} \]

%     \item Licenses are consolidated if the cosine similarity is 0.60 or greater:
%     \[ \text{If } C(E_i, E_j) \geq 0.60, \text{ then licenses } i \text{ and } j \text{ are consolidated.} \]
% \end{enumerate}

% After consolidating licenses, the licenses were then given to an LLM that had been prompted with the information in Table \ref{tab:licenses}, in order to be classified.
% Once every license had been categorized, the count of each category was summed.

% % \begin{itemize}
% %     \item Permissive license: This type of license does not require changes to existing code to be published under the same license as long as they include a copy of the license and attribution to the original authors in the copies or derivative works. Some of the instances of permissive licenses are the Apache License, the BSD License, the MIT License,  and Version 2.0 of the Artistic License.
    
% %     \item Weak copyleft license: This type allows users to change the source code into proprietary application/software, as long as the source code is made available under the same license. Code using the existing code does not have to be published under the same license. Some of the instances of weak copyleft licenses include the Mozilla Public License (MPL), the Lesser GNU Public License (LGPL), and the Eclipse Public License (EPL).
    
% %     \item Strong copyleft license: This is the most restrictive type. Code using the existing code must be published under the same license. Examples of strong copyleft licenses include GNU General Public License (GPL) and GNU Affero General Public License (AGPL).
    
% %     \item Public: This type is the least restrictive type. When the repository is of a public license type, use of the material is made free from restrictions from copyright or database laws, so that others may freely build upon the work, to the full extend possible. "No Rights Reserved". An example of a public license is the CC0 Public Domain License, found here: https://creativecommons.org/public-domain/cc0/
    
% %     \item No License: Without a license, in the case of software typically adherent to the default rules stated by the terms of service if code is located in an hosting platform such as GitHub or Hugging Face (see 7.2 for a further into no license as applicable to this study). 

% %     \item Other: None of the above, these licenses are not the focus of this study, and are not a significant part of our dataset.

% % \end{itemize}


% \subsection{\ctp}
% To measure \ctp relationships, the reach of users was examined.
% \subsubsection{User Reach}
% User reach was found by simply summing the number of packages that a maintainer had contributed to at some point in time, or owned.
% It was calculated as follows:

% Let $P_{contributed}$ be the set of packages a user has contributed to, and $P_{owned}$ be the set of packages owned by the user.
% The User's Reach, $U_{\text{reach}}$, avoiding double counting of packages that are both contributed to and owned, is given by the formula:

% \[
% U_{\text{reach}} = |P_{contributed} \cup P_{owned}|
% \]

% Here, $|A \cup B|$ represents the cardinality of the union of sets $A$ and $B$, which includes all unique packages either contributed to or owned by the user, without double counting any overlap.


% \subsection{\rtp}
% To measure \rtp relationships, the popularity of top packages was examined.
% \subsubsection{Popularity}
% Popularity is measured by looking at the change in top packages over time for each registry.
% In order to obtain the historical data, previous dumps of the Packages dataset were obtained dating back to August 2022.
% However, the earliest snapshot that contain download information was in October 2022.
% For HuggingFace, a dataset with historical data from June 2022 was used, along with PTMTorrent, a previous iteration of PeaTMOSS with data from May 2023, and a current snapshot of HuggingFace from April 2024.

% The turnover for each registry is defined as follows:

% Let $S_{\text{current}}$ be the set of top 1000 packages in the current snapshot, $S_{\text{last}}$ be the set of top 1000 packages in the last snapshot, and $S_{\text{history}}$ be the set of packages that have appeared in any snapshot before the last snapshot. We categorize the packages in $S_{\text{current}}$ into three categories:

% \begin{enumerate}
%     \item \textbf{Returning:} Packages that were once in the top 1000 ($S_{\text{history}}$), weren't in $S_{\text{last}}$, but are in $S_{\text{current}}$.
%     \begin{equation}
%     \text{Returning} = |(S_{\text{history}} \setminus S_{\text{last}}) \cap S_{\text{current}}|
%     \end{equation}
    
%     \item \textbf{Newcomers:} Packages in $S_{\text{current}}$ that have never been in any previous snapshot.
%     \begin{equation}
%     \text{Newcomers} = |S_{\text{current}} \setminus (S_{\text{history}} \cup S_{\text{last}})|
%     \end{equation}
    
%     \item \textbf{Remained:} Packages that were in both $S_{\text{last}}$ and $S_{\text{current}}$.
%     \begin{equation}
%     \text{Remained} = |S_{\text{last}} \cap S_{\text{current}}|
%     \end{equation}
% \end{enumerate}

% The count of packages in categories Remained, Newcomers, and Returning were graphed for each snapshot.

% % \subsubsection{Version Management}
% % Measuring Technical Lag will begin by utilizing the zipped GitHub repositories that we identified were repositories that reused PTMs.
% % In each repository, the signature of reuse will be extracted and used to augment the dataset.
% % Then, each signature will be evaluated to examine whether or not it pins to a specific version of the model.
% % If it does pin, then the commit history of the repository will be examined to determine when, if ever, the version pinned to was updated.
% % The original dependency graph will also be augmented using the "hf\_commit" table to evaluate when commits were made to the model in order to measure the Technical Lag.
% % Technical Lag will be measured as a whole, as well as on a model and architecture basis.

\section{Methods}
% What follows are the methods used to generate data for comparison between traditional software registries (\npm and \pypi) and HuggingFace.

% \JD{You must also explain the comparison itself. How will you decide whether PTM registry is similar or different from traditional? What threshold or measure will you use?}
% \JD{Do you have a hypothesis? State it clearly.}
We adopt a systematic framework to measure both the qualitative and quantitative attributes of traditional software registries (\npm and \pypi) and HuggingFace.
To assess similarities or distinctions, we leveraged a comprehensive suite of metrics describing package interdependency networks and patterns of reuse.
These metrics serve to quantify critical aspects, facilitating a cross-registry comparison.
The criteria for establishing similarity or divergence begins with an initial visual analysis, subsequently eventually corroborated through comparative analytical techniques to ensure a robust, evidence-based evaluation \cite{bobrovitz_comparison_1998, park_visual_1990}.
As of the time of writing, the statistical tests are still in process of being performed, however the obvious visual differences suggest our findings are significant.
% To assess whether HuggingFace is similar to or distinct from traditional registries, we employed a set of metrics encompassing package interdependency networks, contributor influence, and reuse patterns.
% These metrics quantified these key components to allow for comparison across registries.
% The decision criteria for similarity or difference will be based on visual analysis that is eventually supported by comparative analysis techniques such as t-tests.
% The decision criteria for similarity or difference will be based on statistical significance thresholds determined through comparative analysis techniques such as t-tests or effect size measurements, ensuring that observed differences are not merely by chance.

We have a clear hypothesis: \textit{\hypothesis}.
We expect every metric to demonstrate an obvious difference between \hf and traditional software registries.
% This hypothesis seeks to explore the extent to which the unique characteristics of PTMs—arising from their development, deployment, and use cases—translate into observable differences in registry dynamics when compared to traditional software ecosystems.
% Our analysis aims to test this hypothesis through empirical data, offering insights into the implications of these differences for developers, users, and the broader software engineering community

\subsection{Dataset}
There exist several datasets that capture information about HuggingFace \cite{jiang2023ptmtorrent, ait2023hfcommunity}.
% \TODO{[Other dataset]}.
After review of several datasets, we decided to use the PeaTMOSS deataset \cite{jiang_peatmoss_2024}.
The model metadata, the model relationships, and downstream relationships with GitHub repositories captured within the dataset allowed us to compare HuggingFace to traditional software registries.
Through the course of performing analysis using PeaTMOSS, I made several improvements to the dataset to increase its completeness.
% PeaTMOSS is a dataset that captures the metadata of 281,638 Pre-Trained Models hosted on HuggingFace and PyTorch, and connects them to 28,575 GitHub repositories that reuse PTMs, creating 44,337 mappings from 15,129 downstream GitHub repositories to 2,530 PTMs. \cite{jiang_peatmoss_2024}.
% PeaTMOSS also contains 59,011 Discussions from HuggingFace, as well as 827,856 Pull Requests and 631,007 Issues from GitHub. \cite{jiang_peatmoss_2024}
% PeaTMOSS was originally created to facilitate work examining PTM packages across multiple model zoos \cite{jiang_ptmtorrent_2023}.
% The rapid emergence and dominance of HuggingFace and PyTorch as platforms for PTM reuse, as well as the richness of metadata on the HuggingFace platform compared to all other platforms resulted in a reduction of scope to focus entirely on HuggingFace and PyTorch \cite{jiang_peatmoss_2023}.
% The original Model Zoo metadata was eventually augmented with downstream GitHub repositories that reused PTMs from either HuggingFace or PyTorch, in order to create a dataset that contained information about both model contributors and users \cite{jiang_peatmoss_2023}.
% Artifacts related to model contribution (HuggingFace discussions) and downstream reuse (GitHub Issues and Pull Requests) were also captured in the dataset \cite{jiang_peatmoss_2023}.
% The HuggingFace metadata was later augmented using a Large Language Model to further extract details from the relatively unstructured metadata format of HuggingFace model cards \cite{jiang_peatmoss_2024}.
% The significant amount and quality of data available in PeaTMOSS allows for the calculation of metrics originally used to measure traditional software registries.


% \subsection{\ctp}
% To measure \ctp relationships, the reach of users was examined.
% \subsection{User Reach}
% User reach was found by simply summing the number of packages that a maintainer had contributed to at some point in time, or owned.
% It was calculated as follows:

% Let $P_{contributed}$ be the set of packages a user has contributed to, and $P_{owned}$ be the set of packages owned by the user.
% The User's Reach, $U_{reach}$, avoiding double counting of packages that are both contributed to and owned, is given by the formula:

% \begin{equation}
%     U_{reach} =\|P_{contributed} \cup P_{owned}\|         
% \end{equation}

% Here, $\|A \cup B\|$ represents the cardinality of the union of sets $A$ and $B$, which includes all unique packages either contributed to or owned by the user, without double counting any overlap.

% \subsection{\ptp}
\subsection{Dependent Packages}
% To measure \ptp relationships, dependencies were examined.
In the context of PTMs, dependencies are not maintained as ongoing connections to other PTMs but rather as specific checkpoints from which a model has evolved.
This conceptualization is aligned with the impact of dependencies observed in traditional software.
In traditional software ecosystems, a dependency introduces several factors: it enables the continuation of functionality from the dependent package, but it also introduces potential security risks; vulnerabilities in an upstream package can propagate to all dependent packages.
Similarly, for PTMs, a model checkpoint carries forward both the functionality and any inherent security risks of the model at that point.
Therefore, model checkpoints have been designated as the equivalent of dependencies for PTMs, reflecting the functional and security implications typical in traditional software dependencies.

% In the context of PTMs, dependencies exist not as a persistent connection to another PTM, but as a checkpoint from which a model was taken from.
% This definition is been chosen because of the functional effects of a dependency in traditional software.
% In traditional software, a dependency carries with its several considerations, firstly you can you continue to take on the functionality of the  package.
% Second of all, you also incur a security risk in that if a vulnerability is found in a upstream package, that vulnerability is also present in your package.
% Since checkpoint that model is trained from carry on the functionality of that model, as well as the security risks present in that model model checkpoint were selected as the definition of dependency for PTMs.
% As a result, the idea of a dependency tree remains the same, with the only difference being the nature of a dependency.

In the PeaTMOSS dataset, the "model\_to\_base\_model" table links PTMs ("model") to their original "base model" from which they were derived.
This table, established using the DARA pipeline as detailed in \cite{jiang_peatmoss_2024}, facilitates the tracking of model lineages.
For PTMs, the count of dependents is determined by the frequency with which a PTM is referenced as a "base model" within this table.
Conversely, the number of dependencies a PTM has is gauged by the occurrences of it appearing as a "model."
\begin{itemize}
    \item \textbf{Count of Dependents} for a PTM is calculated by:
    \begin{equation}
    \text{Dependents}_{\text{PTM}}(m) = \|\{ x \in \text{model\_to\_base\_model} : \text{base\_model} = m \}\|
    \end{equation}
    where \( m \) represents a specific PTM.

    \item \textbf{Count of Dependencies} for a PTM is determined by:
    \begin{equation}
    \text{Dependencies}_{\text{PTM}}(m) = \|\{ x \in \text{model\_to\_base\_model} : \text{model} = m \}\|
    \end{equation}
    where \( m \) represents a specific PTM.
\end{itemize}

In the context of traditional software, the Ecosyste.ms Packages dataset's "Packages" table records the number of direct dependents for each package as "dependent\_packages\_count".
To assess upstream dependencies, the "dependencies" and "versions" table are utilized.
"dependencies" enumerates the packages that a specific version of a package depends upon.
"versions" describes the versions of a package that exist.
Here, a package's dependency count is derived from the number of times a version of it is listed as a dependent package within this table.

\begin{itemize}
    \item \textbf{Count of Direct Dependents:}
    \begin{equation}
    \text{Dependents}(p) = \text{dependent\_packages\_count}(p)
    \end{equation}
    where \( p \) represents a specific package. This count is directly recorded in the ``Packages'' table in the column "dependent\_packages\_count".

    \item \textbf{Count of Dependencies:}
    To determine the dependencies for a package, two tables are used: the ``dependencies'' table, which enumerates the packages that a specific version of a package depends upon, and the ``versions'' table, which describes the versions of a package that exist.
    
    The count of dependencies, derived from how often a version of a package is listed as a dependency in the ``dependencies'' table, is calculated as:
    \begin{equation}
    \text{Dependencies}(p) = \| \{x \in \text{dependencies} : \text{dependent\_package} = p\} \|
    \end{equation}
    where \( p \) represents a specific package, and ``dependent\_package'' refers to entries in the ``dependencies'' table where \( p \) is listed as a dependency.
\end{itemize}


% In the PeaTMOSS dataset, the table "model\_to\_base\_model" connects PTM "model"s to the original "base model" that they diverged from.
% This table was created using the DARA pipeline, as mentioned in \cite{jiang_peatmoss_2024}.
% For PTMs, the number of dependents is found by counting the number of times a PTM appears as a "base model" in the table.
% Looking upstream at the number of dependencies a PTM has, the number of times a PTM appears as a "model" in the table is used.

% For traditional software, the Ecosyste.ms Packages dataset has a "Packages" table, which includes information such as the number of direct dependents of a package.
% Looking upstream, the table "versions" is used, which describes the specific versions of other packages a package includes as dependencies.
% The number of times a package appears in this table as a dependent package is used for the number of dependenies.

% The count are generated as follows:
% The number of dependent packages ($D_p$) is the number of direct dependents ($N_d$) that a package has:
% \begin{equation}
% D_p = N_d
% \end{equation}

% The number of dependent packages for a PTM ($D_{ptm}$) is the number of models that use it as a checkpoint to train from ($M_c$):
% \begin{equation}
% D_{ptm} = M_c
% \end{equation}

% \subsection{\ptr}
% To measure \ptr relationships, dependent repositories and software licenses were examined.
% \subsection{Licenses}
% Licenses are categorized as shown in \ref{tab:licenses}.
% The raw licenses for each platform are available in both the Packages and PeaTMOSS datasets.
% For each platform, the licenses from the top 10\% of packages were gathered, along with their frequency.
% The licenses were then consolidated based on the embeddings generated, in order to simplify classification.

% Licenses were approached this way because of the lack of standardization in reporting practices for software licenses.
% This resulted in a large amount and variety of raw license data.
% As an example, PyPi had 9,340 different licenses within its top 10\% of packages, with licenses such as
% Apache 2.0, Apache Software License, Apache License 2.0, Apache-2.0, "Apache License, Version 2.0", Apache, and Apache License Version 2.0 all being counted differently.
% Using this method, the number of unique licenses on PyPi was consolidated down to 400, which allowed for a more in-depth manual review of license classifications.

% While it has not been done specifically in the realm of license names, prior work has used embeddings compared pair-wise using cosine similarity to classify things \cite{mathur_putting_2019, zhang_bertscore_2019, kim_evaluating_2022, quan_efficient_2019}.
% After doing it this way and manually reviewing, I found that the consolidation was \TODO{XX\%} effective.

% This consolidation was done as follows:

% % \JD{It is unclear why you are doing it this way as opposed to a more formal/sound approach. Give some rationale for the use of LLMs and cosine embeddings. (What else did you consider? Why did you do it this way? Has anyone else done it this way? Why doesn't other people's approach work for you?)}

% Given a series of software licenses, for each license $L_i$, the process is as follows:

% \begin{enumerate}
%     \item Obtain the first up to 40 characters of each software license $L_i$:
%     \[ L_{i,40} = \text{first 40 characters of } L_i \]

%     \item Generate embeddings for each license excerpt $L_{i,40}$:
%     \[ E_i = E(L_{i,40}) \]
%     Where $E_i$ is the embedding for the $i^{th}$ license's excerpt.

%     \item Compute the cosine similarity between embeddings $E_i$ and $E_j$ for licenses $i$ and $j$:
%     \[ C(E_i, E_j) = \frac{E_i \cdot E_j}{\|E_i\|\|E_j\|} \]

%     \item Licenses are consolidated if the cosine similarity is 0.60 or greater:
%     \[\text{ If } C(E_i, E_j) \geq 0.60,  \text{then licenses } i \text{ and } j  \text{ are consolidated.} \]
% \end{enumerate}

% After consolidating licenses, the licenses were then given to an LLM that had been prompted with the information in Table \ref{tab:licenses}, in order to be classified.
% Once every license had been categorized, the count of each category was summed.

\subsection{Dependent Repositories}
The number of dependent repositories ($R_d$) is the number of repositories that directly include the package ($R_i$), whether it is traditional software or a PTM.
% PeaTMOSS stores this information in the "model\_to\_reuse\_repository" table, which connects upstream models to downstream GitHub Repositories that reuse them.
% The count of dependent repositories is the number of times a model is connected to a repository through this table.

The number of dependent repositories, denoted as \(R_d\), for a PTM is calculated by counting the connections between models and repositories in the "model\_to\_reuse\_repository" table. This can be expressed as:
\begin{equation}
R_d = \| \{x \in \text{model\_to\_reuse\_repository} : \text{model} = m\} \|
\end{equation}
where \( m \) represents a specific PTM.

In the context of traditional software, the count of dependent repositories \(R_d\) for a package is directly recorded in the "Packages" table under the column "dependent\_repos\_count". This can be formalized as:
\begin{equation}
R_d(p) = \text{dependent\_repos\_count}(p)
\end{equation}
where \( p \) represents a specific software package.


% \subsection{\rtp}
% To measure \rtp relationships, the popularity of top packages was examined.
\subsection{Popularity}
Popularity is measured by looking at the change in top packages over time for each registry.
In order to obtain the historical data, previous dumps of the Packages dataset were obtained dating back to August 2022.
However, the earliest snapshot that contain download information was in October 2022.
For HuggingFace, a dataset with historical data from June 2022 was used, along with PTMTorrent, a previous iteration of PeaTMOSS with data from May 2023, and a current snapshot of HuggingFace from April 2024.

The turnover for each registry is defined as follows:

Let $S_{current}$ be the set of top 1000 packages in the current snapshot, $S_{last}$ be the set of top 1000 packages in the last snapshot, and $S_{history}$ be the set of packages that have appeared in any snapshot before the last snapshot. We categorize the packages in $S_{current}$ into three categories, and evaluate the number of packages in each set:

\begin{enumerate}
    \item \textbf{Remained:} Packages that were in both $S_{last}$ and $S_{current}$.
    \begin{equation}
    \text{Remained} = S_{last} \cap S_{current}
    \end{equation}

    \item \textbf{Returning:} Packages that were once in the top 1000 ($S_{history}$), weren't in $S_{last}$, but are in $S_{current}$.
     % \JD{The set notation is cardinality (size of the set), but the definition in prose is the set itself. Which is it? You might need to change the prose to ``Number of packages...'' for this definition and the next two}
    \begin{equation}
    \text{Returning} = (S_{history} \setminus S_{last}) \cap S_{current}
    \end{equation}
    
    \item \textbf{Newcomers:} Packages in $S_{current}$ that have never been in any previous snapshot.
    \begin{equation}
    \text{Newcomers} = S_{current} \setminus (S_{history} \cup S_{last})
    \end{equation}
\end{enumerate}

The count of packages in the Remained, Newcomers, and Returning sets were graphed for each snapshot.

% \subsubsection{Version Management}
% Measuring Technical Lag will begin by utilizing the zipped GitHub repositories that we identified were repositories that reused PTMs.
% In each repository, the signature of reuse will be extracted and used to augment the dataset.
% Then, each signature will be evaluated to examine whether or not it pins to a specific version of the model.
% If it does pin, then the commit history of the repository will be examined to determine when, if ever, the version pinned to was updated.
% The original dependency graph will also be augmented using the "hf\_commit" table to evaluate when commits were made to the model in order to measure the Technical Lag.
% Technical Lag will be measured as a whole, as well as on a model and architecture basis.

% \section{Results}
% \subsection{\ptp}
% \subsubsection{Dependent Packages}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.45\textwidth]{dep_packages.png}
%     \caption{
%     The Top 10\% of Depended on Packages for representative traditional software package registries(NPM in Blue, PyPi in Orange) and the representative PTM registry HuggingFace. This figure ranks by the number of inter-package dependencies. Both NPM and PyPi demonstrate a similar curve and drop-off of dependents, while HuggingFace experiences an incredibly rapid drop off.
%     }
%     \label{fig:dep_packages}
% \end{figure}

% As shown in Figure \ref{fig:dep_packages}, there is a clear difference between the different package registries.
% Both traditional software package registries have a small set of packages that are widely depended on, then a larger set of packages that are depended on by a medium to small set of packages.
% In contrast to this, HuggingFace has a tiny amount of PTMs that are depended on by some other PTMs, but then immediately drops off to packages with singular dependencies, before finally reaching PTMs with no dependencies, a full 9 percentile points before PyPi does.
% This suggests that there is much less inter-package dependencies than other platforms.
% In order to further explore this phenomenon, I will take a look at the number of indirect dependencies a package on each platform to further characterize each platform's inter-package relationships.
% However, the immediate implication of this indicates that the HuggingFace ecosystem is much more resilient to attacks, and less likely to propagate exploits to a large number of packages.

% \subsection{\ptr}
% \subsubsection{Dependent Repositories}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.45\textwidth]{dep_repos.png}
%     \caption{
%     The Top 10\% of Depended on Packages for representative traditional software package registries (NPM in Blue, PyPi in Orange) and the representative PTM registry HuggingFace. This figure ranks by the number of downstream repositories that include the package. Both NPM and PyPi demonstrate a similar curve and drop-off of dependents, while HuggingFace experiences an incredibly rapid drop off.
%     }
%     \label{fig:dep_repos}
% \end{figure}

% As shown in Figure \ref{fig:dep_repos}, there is a clear difference between the different package registries.
% Both traditional software package registries have a small but significant amount of packages that are widely used downstream.
% This then gives way to a large amount of packages that are moderately used downstream, then an even larger amount of packages that are rarely used downstream.
% HuggingFace starts off similarly with a small set of PTMs that are used widely downstream.
% However, outside of this small set, the usage drops immediately into the single digits, before eventually dropping to 0 before reaching the 99th percentile of PTMs.

% \subsubsection{Licenses}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.95\textwidth]{licenses.png}
%     \caption{
%     Distribution of Software License Categories across NPM, PyPi, and HuggingFace.
%     NPM is the most explicitlty permissive platform, but all three platforms license packages permissively.
%     There are some differences, however.
%     While it appears as though PyPi is the least permissive platform, a large reason for that is the significant number of unlicensed packages.
%     When considered as Permissive Licenses, PyPi is more permissive as a platform than HuggingFace is. 
% }
%     \label{fig:license}
% \end{figure*}

% As shown in Figure \ref{fig:license}, there does not seem to be a clear pattern of license selection across traditional software and PTMs.
% Interesting to note is that HuggingFace has more than 7\% of its models put into the public domain, compared to 0.35\% of PyPi and 0.0\% of NPM packages.
% Further analysis needs to be performed to characterize this metric.
% Rather than looking at only the number of packages that use each license, I will examine the relative popularity in terms of downloads, dependent packages, and dependent repositories of each license category.
% Additionally, I will manually review both the PyPi and HuggingFace licenses to determine if they need to be re-classified.

% \subsection{\ctp}
% \subsubsection{Contributor Reach}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{contributors.png}
%     \caption{
%     The top 10\% of Contributors on NPM, PyPi, and HuggingFace organized by the number of Packages they either own or contribute to. Note that the representative traditional software package registries (NPM and PyPi and Blue and Orange respectively) and the representative PTM registry (HuggingFace in green) both demonstrate the same exponential curve shape. The shape of these curves indicates that there is a small concentration of ``power users`` that have a significant reach and influence on the registries. This group of power users appears to be proportional to the registries as well, since the drop off appears to occur at around the same percentile across all three registries.
%     % \JD{The current prose is too much of the form ``It is obvious...any fool can see that...''. Assume the reader is tired and be gentle. Walk them through the figure, using plain English and implying the legend as you go. Here is an example. ``Note that in the representative traditional software package registries, NPM and PyPI, the level of turnover is low. Most of the top-1000 packages remain the same across the snapshots in time we examined, as indicated by the large proportion taken up by the blue bars in the second and third snapshots. In contast, in the representative PTM registry, HuggingFace, there is a higher level of turnover...''}
% }
%     \label{fig:contributors}
% \end{figure}

% Interestingly enough, it appears that each registry has a similar amount of user reach, as shown in Figure \ref{fig:contributors}.
% Again, however, this may not tell the full story of user reach across each platform, so I will continue to characterize this metric by examining the reach of contributors in terms of downloads, dependent packages, and dependent repositories, to see if there is a clear pattern that emerges there.
% I will also look at this metric from the point of view of the packages, to examine the average number of contributors to a specific package.
% This will provide interesting implications about the level of cooperation between maintainers across the various platforms.

% \subsection{\rtp}
% \subsubsection{Turnover}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{turnover.png}
%     \caption{
%     The turnover of the top-1000 Packages on HuggingFace, NPM, and PyPi. Note that in traditional software package registries NPM and PyPi, the level of turnover is low. Most of the Top 1000 packages remain the same across the snapshots we examined, as indicated by the large blue bars in the second and third snapshots. In contrast, in the representative PTM registry HuggingFace, there is a much higher level of turnover, shown by the orange bar being larger than the blue bar in the second and fourth snapshots. Additionally, HuggingFace has a much larger amount of packages re-enter the Top 1000 as shown by the larger green bars in the second and fourth snapshot compared to NPM and PyPi, who have almost no returners, as shown by the relative lack of green bars. 
%     % \JD{The current prose is too much of the form ``It is obvious...any fool can see that...''. Assume the reader is tired and be gentle. Walk them through the figure, using plain English and implying the legend as you go. Here is an example. ``Note that in the representative traditional software package registries, NPM and PyPI, the level of turnover is low. Most of the top-1000 packages remain the same across the snapshots in time we examined, as indicated by the large proportion taken up by the blue bars in the second and third snapshots. In contast, in the representative PTM registry, HuggingFace, there is a higher level of turnover...''}
%     % \JD{I agree the blue vs orange is different, but the green looks similar between PyPI and HuggingFace. Is that significant enough to emphasize?}
% }
%     \label{fig:turnover}
% \end{figure*}
    

% Figure \ref{fig:turnover} shows very clear differences between traditional software and PTM registries.
% While it can be seen that the most popular packages remained the most popular on traditional software registries like NPM and PyPi, HuggingFace experiences a large amount of turnover at the top, seeing a total of 2535 packages enter the Top 1000 compared to 1429 on PyPi and just 1127 for NPM.
% This suggests that a package has a much shorter "lifespan" on the PTM platform than on traditional software registries.
% I will continue to examine this metric by looking at the average life of packages that enter into and exit out of the top thousand to see if it is new packages that are briefly entering and then leaving or if it is more established packages that are leaving the top 1000.
% The packages captured by this metric will also be examined to see which maintainers enter into and remain within the top 1000 both in terms of number of packages and just any presence at all.

% \section{Analysis}

% % \JD{This is too close to your findings. The conclusion must walk us from the specifics back out to the general world.}

% \subsection{\ptp}
% \subsubsection{Dependent Packages}
% As shown in Figure \ref{fig:dep_packages} HuggingFace has a much lower amount of connections between packages than NPM and PyPi.
% This would indicate that PTMs rely less on the synthesis of multiple PTMs together to create new functionality the way that traditional software does.
% This would indicate that the PTM supply chain has les interconnection between packages, and is less vulnerable to vulnerability propagation.
% It would also indicate that unlike unlike traditional software package development which is often the bundling of function of packages and some extension of that funcion, PTM development is largely the modification of a specific model to fit a new purpose, which matches with previous findings. 

% \subsection{\ptr}
% \subsubsection{Dependent Repositories}
% As shown in Figure \ref{fig:dep_repos}, \hf has a much steeper drop off of package usage compared to NPM and PyPi.
% All of the usage of PTMs is described by the 99th percentile and above of PTMs on \hf.
% This suggests that though there are a large amount of PTMs available on the HuggingFace platform, only a small handful are used downstream.
% It is possible that there is more firect competition among PTMs for selection, and that there is a more objective way to compare performance, resulting in there being a "winning" model that is always selected.

% \subsubsection{Package Licenses}
% As shown in Figure \ref{fig:license} all platforms are similarly permissive with the licensing of their packages.
% This would indicate that although people in general claim that AI and ML need to be regulated and controlled, that the widespread creators of PTMs don't engage with them and restrict them any differently than traditional software users do.

% \subsection{\ctp}
% \subsubsection{User Reach}
% The reach of users displays similar patterns on HuggingFace as it does on traditional software registries, as shown in Figure \ref{fig:contributors}.
% HuggingFace has a small group of users that contribute a lot, then the reach of users quickly falls off.
% NPM and PyPi both show this same phenomemnom.
% As a result, the PTM supply chain is vulnerable to similar kinds of attacks as the traditional supply chain as it pertains to malicious actors.
% These actors have similar widespread reach on the PTM Supply Chain as they o in the traditional supply chain.

% \subsection{\rtp}
% \subsubsection{Package Selection}
% Figure \ref{fig:turnover} demonstrates that popular packages on HuggingFace have a much greater turnover rate than traditional software packages do on NPM and PyPi.
% In fact, unlike in the other platforms where popular packages become more stable over time, the top packages remained similarly unstable.
% This would indicate that the lifespan of PTM relevance is shorter than the longevity of traditional software package relevance.
% It would also indicate that a traditional software needs are more stable than PTM needs.
% It is possible that since traditional software needs are established, that they change less and so the same packages are needed
% In contrast, it may be that the wide range of domains in which PTMs are applicable means that at different times, different kinds of PTMs are needed.
% This would also be supported by the increased amount of Returning packages on HuggingFace compared to NPM and PyPi.

\section{Results and Analysis}
Findings from this work provide further understanding into how PTM Supply Chains compare to  Traditional Software Supply Chains.
I provide a discussion of observed similarities and differences, and relate possible areas of future work.

% \begin{sidewaystable}
% \centering
% \label{table:results-summary}
% \caption[Results Summary]{
% Summary of Results organized by Dimension
% % \JD{This caption is too short. Please expand it to multiple sentences. For example, is the set of metrics exhaustive? Why these ones?}
% }
% \begin{tabular}{m{0.12\linewidth} m{0.12\linewidth} m{0.1\linewidth} m{0.3\linewidth} m{0.3\linewidth}} 
% \toprule
% \textbf{Dimension} & \textbf{Relationship} & \textbf{Metric} & \textbf{Traditional Software Pattern} & \textbf{PTM Pattern}  \\ 
% \midrule
% Contribution & Contributor-to-Package & User Reach & A core group of users have a high amount of reach, with a slow, exponential decay of reach as less influential users are measured & A core group of users have a high amount of reach, with a slow, exponential decay of reach as less influential users are measured \\ % User Reach
% \midrule
% Evolution & Package-to-Package & Dependency Amount & A small group of packages have a large number of dependents, with slow, exponential decay as less depended on packages are measured. In the other direction, packages rely on a large amount of dependencies. & A small group of PTMs are depended on, but once that group is moved past, PTMs are not depended on. In the other direction, PTMs have, for the most part, exactly 1 dependency. \\ % Dependency
% \midrule
% Reuse  & Package-to-Reuser & Licenses & Package licenses are generally Permissive, with a minor portion having proprietary licenses. & Package licenses are generally Permissive, with a significant portion having proprietary licenses, and a minor amount being open-source.  \\ % License
% \addlinespace[10pt]
%  &  & Downstream Projects & A small group of packages are reused by a large number of downstream projects. Once this group of packages is moved past, there is an exponential decay of reuse with a long tail. & A small group of PTMs are reused by a large amount of downstream projects. Once this group of PTMs is moved past, there are is almost no downstream project reuse. \\ % License
% \addlinespace[10pt]
%  & Reuser-to-Package & Popularity & A small group of packages is the most popular with a slow exponential decay as packages become less popular. The most popular packages don't experience much turnover & A small group of PTMs is the most popular with a slow exponential decay that transforms into a fast exponential decay as PTMs become less popular. The most popular PTMs experience high turnover \\ % Popularity
%                               % & Technical Lag        & How long does it take to utilize new updates   & How trusted are package updates           & NPM, PyPi, Maven, Cargo                                          & \cite{zerouali_formal_2019, pinckney_large_2023, wittern_look_2016, zerouali_empirical_2018, decan_evolution_2018, stringer_technical_2020} \\ % Technical Lag
% \bottomrule
% \end{tabular}
% \end{sidewaystable}

\begin{table*}
\centering
\label{table:results-summary}
\caption[Results Summary]{
Summary of Results organized by Dimension
% \JD{This caption is too short. Please expand it to multiple sentences. For example, is the set of metrics exhaustive? Why these ones?}
}
\begin{tabular}{m{0.15\linewidth} m{0.15\linewidth} m{0.3\linewidth} m{0.3\linewidth}} 
\toprule
\textbf{Dimension} & \textbf{Metric} & \textbf{Traditional Software Pattern} & \textbf{PTM Pattern}  \\ 
\midrule
Evolution & Dependent Packages & A small group of packages have a large number of dependents, with slow, exponential decay as less depended on packages are measured. & A small group of PTMs are depended on, but once that group is moved past, PTMs are not depended on. \\ % Dependency
\addlinespace[10pt]
 & Package Dependencies & In the other direction, packages rely on a large amount of dependencies. & In the other direction, PTMs have, for the most part, exactly 1 dependency. \\ % Dependency
\midrule
Reuse & Downstream Projects & A small group of packages are reused by a large number of downstream projects. Once this group of packages is moved past, there is an exponential decay of reuse with a long tail. & A small group of PTMs are reused by a large amount of downstream projects. Once this group of PTMs is moved past, there are is almost no downstream project reuse. \\ % Downstream Reuse
\addlinespace[10pt]
 & Popularity & A small group of packages is the most popular with a slow exponential decay as packages become less popular. The most popular packages don't experience much turnover & A small group of PTMs is the most popular with a slow exponential decay that transforms into a fast exponential decay as PTMs become less popular. The most popular PTMs experience high turnover \\ % Popularity
                              % & Technical Lag        & How long does it take to utilize new updates   & How trusted are package updates           & NPM, PyPi, Maven, Cargo                                          & \cite{zerouali_formal_2019, pinckney_large_2023, wittern_look_2016, zerouali_empirical_2018, decan_evolution_2018, stringer_technical_2020} \\ % Technical Lag
\bottomrule
\end{tabular}
\end{table*}

% \subsection{Theme 1: Package Contribution}\label{sec:package-contribution-results}
% \subsubsection{RQ 1.1: \ctp}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{contributors.png}
%     \caption[The top 10\% of Contributors on NPM, PyPi, and HuggingFace organized by the number of Packages they either own or contribute to]{
%     The top 10\% of Contributors on NPM, PyPi, and HuggingFace organized by the number of Packages they either own or contribute to. Note that the representative traditional software package registries (NPM and PyPi and Blue and Orange respectively) and the representative PTM registry (HuggingFace in green) both demonstrate the same exponential curve shape. The shape of these curves indicates that there is a small concentration of ``power users`` that have a significant reach and influence on the registries. This group of power users appears to be proportional to the registries as well, since the drop off appears to occur at around the same percentile across all three registries.
%     % \JD{The current prose is too much of the form ``It is obvious...any fool can see that...''. Assume the reader is tired and be gentle. Walk them through the figure, using plain English and implying the legend as you go. Here is an example. ``Note that in the representative traditional software package registries, NPM and PyPI, the level of turnover is low. Most of the top-1000 packages remain the same across the snapshots in time we examined, as indicated by the large proportion taken up by the blue bars in the second and third snapshots. In contast, in the representative PTM registry, HuggingFace, there is a higher level of turnover...''}
% }
%     \label{fig:contributors}
% \end{figure}

% \ul{Contributor Reach:}\label{sec:contributor-reach} Interestingly enough, it appears that each registry has a similar amount of user reach, as shown in Figure \ref{fig:contributors}.
% Again, however, this may not tell the full story of user reach across each platform, so I will continue to characterize this metric by examining the reach of contributors in terms of downloads, dependent packages, and dependent repositories, to see if there is a clear pattern that emerges there.
% I will also look at this metric from the point of view of the packages, to examine the average number of contributors to a specific package.
% This will provide interesting implications about the level of cooperation between maintainers across the various platforms.
% The reach of users displays similar patterns on HuggingFace as it does on traditional software registries, as shown in Figure \ref{fig:contributors}.
% HuggingFace has a small group of users that contribute a lot, then the reach of users quickly falls off.
% NPM and PyPi both show this same phenomemnom.
% As a result, the PTM supply chain is vulnerable to similar kinds of attacks as the traditional supply chain as it pertains to malicious actors.
% These actors have similar widespread reach on the PTM Supply Chain as they o in the traditional supply chain.

\subsection{RQ 1: Package Evolution}\label{sec:package-evolution-results}
\subsubsection{Dependent Packages}\label{sec:package-interdep}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth]{archived/dep_packages.png}
    \caption[The Top 10\% of Depended on Packages for representative traditional software and PTM registries]{
    The Top 10\% of Depended on Packages for representative traditional software package registries(NPM in Blue, \pypi in Orange) and the representative PTM registry HuggingFace. This figure ranks by the number of inter-package dependencies. Both NPM and \pypi demonstrate a similar curve and drop-off of dependents, while HuggingFace experiences an incredibly rapid drop off.
    }
    \label{fig:dep_packages}
\end{figure}

% \ul{Package Interdependencies}\label{sec:package-interdep} 
As shown in Figure \ref{fig:dep_packages}, there is a clear difference between the different package registries.
Both traditional software package registries have a small set of packages that are widely depended on, then a larger set of packages that are depended on by a medium to small set of packages.
In contrast to this, HuggingFace has a tiny amount of PTMs that are depended on by some other PTMs, but then immediately drops off to packages with singular dependencies, before finally reaching PTMs with no dependencies, a full 9 percentile points before \pypi does.
This suggests that there is much less inter-package dependencies than other platforms.
In order to further explore this phenomenon, I will take a look at the number of indirect dependencies a package on each platform to further characterize each platform's inter-package relationships.
However, the immediate implication of this indicates that the HuggingFace ecosystem is much more resilient to attacks, and less likely to propagate exploits to a large number of packages.
As shown in Figure \ref{fig:dep_packages} HuggingFace has a much lower amount of connections between packages than NPM and \pypi.
This would indicate that PTMs rely less on the synthesis of multiple PTMs together to create new functionality the way that traditional software does.
This would indicate that the PTM supply chain has les interconnection between packages, and is less vulnerable to vulnerability propagation.
It would also indicate that unlike unlike traditional software package development which is often the bundling of function of packages and some extension of that funcion, PTM development is largely the modification of a specific model to fit a new purpose, which matches with previous findings. 

\subsection{Theme 2: Package Reuse}\label{sec:package-reuse-results}

% \subsubsection{RQ 3.1: \ptr}
% \subsubsection{Package Licenses}\label{sec:esem-licenses:}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.95\textwidth]{licenses.png}
%     \caption[Distribution of Software License Categories across NPM, PyPi, and HuggingFace]{
%     Distribution of Software License Categories across NPM, PyPi, and HuggingFace.
%     NPM is the most explicitlty permissive platform, but all three platforms license packages permissively.
%     There are some differences, however.
%     While it appears as though PyPi is the least permissive platform, a large reason for that is the significant number of unlicensed packages.
%     When considered as Permissive Licenses, PyPi is more permissive as a platform than HuggingFace is. 
% }
%     \label{fig:license}
% \end{figure*}

% % \ul{Package Licenses}\label{sec:esem-licenses:}
% As shown in Figure \ref{fig:license} all platforms are similarly permissive with the licensing of their packages.
% This would indicate that although people in general claim that AI and ML need to be regulated and controlled, that the widespread creators of PTMs don't engage with them and restrict them any differently than traditional software users do.

% As shown in Figure \ref{fig:license}, there does not seem to be a clear pattern of license selection across traditional software and PTMs.
% Interesting to note is that HuggingFace has more than 7\% of its models put into the public domain, compared to 0.35\% of PyPi and 0.0\% of NPM packages.
% Further analysis needs to be performed to characterize this metric.
% Rather than looking at only the number of packages that use each license, I will examine the relative popularity in terms of downloads, dependent packages, and dependent repositories of each license category.
% Additionally, I will manually review both the PyPi and HuggingFace licenses to determine if they need to be re-classified.


\subsubsection{Dependent Repositories:}\label{sec:dependent-repos}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth]{archived/dep_repos.png}
    \caption[The Top 10\% of Depended on Packages for representative traditional software package and PTM registries]{
    The Top 10\% of Depended on Packages for representative traditional software package registries (NPM in Blue, \pypi in Orange) and the representative PTM registry HuggingFace. This figure ranks by the number of downstream repositories that include the package. Both NPM and \pypi demonstrate a similar curve and drop-off of dependents, while HuggingFace experiences an incredibly rapid drop off.
    }
    \label{fig:dep_repos}
\end{figure}

As shown in Figure \ref{fig:dep_repos}, there is a clear difference between the different package registries.
Both traditional software package registries have a small but significant amount of packages that are widely used downstream.
This then gives way to a large amount of packages that are moderately used downstream, then an even larger amount of packages that are rarely used downstream.
HuggingFace starts off similarly with a small set of PTMs that are used widely downstream.
However, outside of this small set, the usage drops immediately into the single digits, before eventually dropping to 0 before reaching the 99th percentile of PTMs.
As shown in Figure \ref{fig:dep_repos}, \hf has a much steeper drop off of package usage compared to NPM and \pypi.
All of the usage of PTMs is described by the 99th percentile and above of PTMs on \hf.
This suggests that though there are a large amount of PTMs available on the HuggingFace platform, only a small handful are used downstream.
It is possible that there is more firect competition among PTMs for selection, and that there is a more objective way to compare performance, resulting in there being a "winning" model that is always selected.

\subsubsection{Package Turnover}\label{sec:turnover}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figs/turnover.png}
    \caption[The turnover of the top-1000 Packages on HuggingFace, NPM, and PyPI]{
    The turnover of the top-1000 Packages on HuggingFace, NPM, and \pypi. Note that in traditional software package registries NPM and \pypi, the level of turnover is low. Most of the Top 1000 packages remain the same across the snapshots we examined, as indicated by the large blue bars in the second and third snapshots. In contrast, in the representative PTM registry HuggingFace, there is a much higher level of turnover, shown by the orange bar being larger than the blue bar in the second and fourth snapshots. Additionally, HuggingFace has a much larger amount of packages re-enter the Top 1000 as shown by the larger green bars in the second and fourth snapshot compared to NPM and \pypi, who have almost no returners, as shown by the relative lack of green bars. 
    % \JD{The current prose is too much of the form ``It is obvious...any fool can see that...''. Assume the reader is tired and be gentle. Walk them through the figure, using plain English and implying the legend as you go. Here is an example. ``Note that in the representative traditional software package registries, NPM and PyPI, the level of turnover is low. Most of the top-1000 packages remain the same across the snapshots in time we examined, as indicated by the large proportion taken up by the blue bars in the second and third snapshots. In contast, in the representative PTM registry, HuggingFace, there is a higher level of turnover...''}
    % \JD{I agree the blue vs orange is different, but the green looks similar between PyPI and HuggingFace. Is that significant enough to emphasize?}
}
    \label{fig:turnover-old}
\end{figure*}
    

Figure \ref{fig:turnover} shows very clear differences between traditional software and PTM registries.
While it can be seen that the most popular packages remained the most popular on traditional software registries like NPM and \pypi, HuggingFace experiences a large amount of turnover at the top, seeing a total of 2535 packages enter the Top 1000 compared to 1429 on \pypi and just 1127 for NPM.
This suggests that a package has a much shorter "lifespan" on the PTM platform than on traditional software registries.
I will continue to examine this metric by looking at the average life of packages that enter into and exit out of the top thousand to see if it is new packages that are briefly entering and then leaving or if it is more established packages that are leaving the top 1000.
The packages captured by this metric will also be examined to see which maintainers enter into and remain within the top 1000 both in terms of number of packages and just any presence at all.

Figure \ref{fig:turnover} demonstrates that popular packages on HuggingFace have a much greater turnover rate than traditional software packages do on NPM and \pypi.
In fact, unlike in the other platforms where popular packages become more stable over time, the top packages remained similarly unstable.
This would indicate that the lifespan of PTM relevance is shorter than the longevity of traditional software package relevance.
It would also indicate that a traditional software needs are more stable than PTM needs.
It is possible that since traditional software needs are established, that they change less and so the same packages are needed
In contrast, it may be that the wide range of domains in which PTMs are applicable means that at different times, different kinds of PTMs are needed.
This would also be supported by the increased amount of Returning packages on HuggingFace compared to NPM and \pypi.

% \section{Discussion and Future Work}
% \subsection{Triangulating results}


% \subsection{Future Work}
% We acknowledge that HuggingFace may be immature as a platform for reuse.
% At the time that the data was taken, HuggingFace had \TODO{X} PTMs, it now has \TODO{Y}.
% As a result, it is possible that the differences in metrics is due to immaturity as a platform, rather than a special difference that sets it apart from traditional software package repositories.
% We leave it for future exploration the examining of these metrics in the context of its age as a platform, and the comparison to the metrics of other traditional software packages at their age.

% \section{Threats to Validity} \label{sec:Threats}

% Every empirical research work is conducted in the real world.
% Gaps between the theoretical concepts and reality, and the ways in which reality is measured, may hamper the validity of the study.
% We relied heavily on prior work, and inherit the shortcomings of those works.
% In addition, this paper explores novel territories, this incurring new threats as well.

% \subsection{Construct}

% \textit{Constructs} are the operationalizations of the concepts measured in this work.
% Here we highlight threats, i.e., ways in which our operationalizations may be invalid.

% % The operationalization of dependency in the pre-trained model context is questionable.
% There may be issues in how well the existing constructs for traditional software supply chains map onto the PTM supply chain.
% The traditional concept of dependency in software packages may not directly apply to PTMs because dependencies in PTMs can manifest differently.
% In traditional software, a dependency can be present in a dev environment, at build, or at runtime.
% Each of these kinds of dependencies ultimately involves incorporating the functionality of a outside package into your own.
% However, the nature of PTMs means that they do not have the same kinds of opportunities for other packages to incorporate into thems.
% PTMs often depend on other models not for functionality but for their pretrained weights or architectures.
% As a result, there is not a direct translation of dependencies from traditional software to PTMs that exists.
% % The construct of licenses is also questionable in particular because the new realm of PTM's could possibly result in new kinds of licenses that aren't properly covered by the pre-existing licensed definitions.

% PTMs have novel attributes compared to traditional software.
% Additionally, the unique functionality that PTMs provide has also given rise to additional ethical and moral considerations compared to traditional software.
% As a result, existing definitions of software licenses may not fully encompass the range of licensing arrangements used for PTMs.
% It's possible that licenses which appear identical through the lens of traditional software licensing may, in fact, differ significantly when considering the impact on a PTM's reuse.
% If so, these ostensibly similar licenses could have distinct implications for the reuse of PTMs, despite being classified under the same category
% As a result, the differences in these licenses would not actually be expressed in the popularity of associated models.

% % Dependency was intentionally chosen in order in a functional comparison.
% % The purpose of dependencies in terms of their outcome and why they were studied, was examined in traditional software, and then the closest definition that would allow for the same attribute that dependency has traditional software was chosen for pre-trained models.
% In order to address our concerns about dependencies, a functional comparison approach was taken.
% A definition of dependencies for PTMs was chosen that mirrors the impact of dependencies in traditional software as closely as possible.
% This approach sought to preserve the conceptual integrity of dependency while adapting it to the unique context of PTMs.
% In the future, a definition of dependency that encompasses PTM attributes such as architecture and framework would also better represent the dependency in a PTM context.

% We do not have a plan to mitigate our concerns about licenses at the moment.

% % particularly the reuse patterns of Pre-Trained Models (PTMs) versus traditional software packages.

% \subsection{Internal}

% \textit{Internal} refers to the strength of association between our causes and outcomes in this work.
% Here we highlight ways in which our results may be inaccurate and unreproducible.

% % Selection of Metrics: The choice and application of metrics to compare traditional software registries with the Hugging Face ecosystem might introduce bias. If the selected metrics inherently favor the characteristics of one ecosystem over another, the results could be skewed.
% % Dataset Completeness and Accuracy: The quality and completeness of the datasets used (PeaTMOSS for PTMs and Packages dataset for traditional software) could influence the study's findings. Missing data, inaccuracies, or biases in these datasets could misrepresent the actual dynamics of the ecosystems studied.
% % Analysis Techniques: The methods used to analyze the datasets and interpret the results must be robust and appropriate for the data. Any limitations in the analytical techniques could lead to incorrect conclusions about the differences between traditional software and PTM registries.
% The choice and application of metrics to compare traditional software registries with the Hugging Face ecosystem might introduce bias.
% Many metrics that come from traditional software were developed for, and applied to a single registry in order to characterize that registry.
% If the selected metrics inherently favor the characteristics of one registry over another, the results could be skewed.

% Another possible issue is the completeness of the datasets used in the study (PeaTMOSS for PTMs and Packages dataset for traditional software).
% These datasets aggregate self-reported metadata from the registries.
% Missing data, inaccuracies, or biases could result in a misrepresentation of the studied registries.
% Additionally, these datsets are ultimately snapshots of inherently volatile platforms.
% As such, it is possible that these snapshots contain results that would be irreproducible with snapshots that were taken just a few months separate.

% % \JD{I don't understand the relevance of the next paragraph?}
% % Additionally, PTMS inherently change the dynamics compared to traditional software.
% % While a traditional software registry provides the source code of a package, PTMs are typically made available through Model Zoos by providing only the model weights and definitions, which are sufficient for reuse.
% % However, they do not include the code and datasets used to develop these models, potentially obscuring crucial information about the model's formation and underlying data.

% To mitigate concerns regarding metric selection, we chose metrics with a proven track record across diverse software platforms, reducing the potential for bias.
% Furthermore, we selected a broad spectrum of registry aspects for measurement, ensuring a comprehensive analysis of the registries in question.

% % Additionally, model zoos are generally unique platforms compared to software registries.
% % Where a traditional software registry provide the source code of the package, Model Zoos just provide the weights and definition of a model, just enough for it to be re-used.
% % They do not provide the code and datasets that were used to create those models, which can obfuscate information about the information of the model.

% \subsection{External}

% \textit{External} refers to the generalizability of our work.
% Here we highlight ways in which our results may not be generalizable.

% % Generalizability to Other Ecosystems: The study focuses on the Hugging Face ecosystem compared to NPM and PyPi. The findings may not be generalizable to other software registries or PTM ecosystems with different characteristics or governance models.
% % Evolving Nature of PTMs and Ecosystems: The rapidly evolving nature of PTMs and their ecosystems might limit the longevity of the study's findings. New trends, technologies, or practices emerging after the study's completion could alter the dynamics of PTM reuse, dependencies, and licensing.
% % Influence of Unexamined Factors: There could be external factors not examined in the study that significantly influence the reuse patterns of PTMs and traditional software. These might include community norms, regulatory changes, or shifts in technology that impact how engineers interact with these ecosystems.

% This study focuses on comparing the Hugging Face ecosystem to NPM and PyPi.
% Existing ecosystems like NPM, PyPi, Cargo, and others have all been studied together to see if they display similar patterns of behaviors~\cite{decan_empirical_2019}.
% It was found that they exhibit general behaviors that are similar, but that there are differences between ecosystems in the degree of those behaviors.
% % \JD{Hmm, the next sentence is a bit odd. The claimed result is that HF is not the same as npm/pypi, so the reader is wondering if we are making a bigger claim --- that HF is not the same as Crates, RubyGems, etc. The next sentence is too vague, customize it to your actual study and claimed findings}
% It is important to acknowledge that our conclusions about the unique nature of HuggingFace, in contrast to NPM and PyPi, may not directly apply to other software registries such as Crates or RubyGems, which could exhibit different characteristics when evaluated using these same metrics.

% The rapidly evolving nature of PTMs and their ecosystems might limit the longevity of the study's findings.
% New trends, technologies, or practices emerging after the study's completion could alter the dynamics of PTM reuse, dependencies, and licensing.
% It is also entirely possible that the trends shown in this study are purely due to the realtively young age of HuggingFace compared to NPM and PyPi.
% HuggingFace was created in 2016, and began to explode in popularity as a platform in 2020.
% For comparison, NPM was created in 2010, and PyPi was created in the early 2000s.
% It may be that as HuggingFace matures as a platform, that the patterns shown here begin to resemble those of their contemporaries, especially when it comes to interpackage dependency networks and the turnover rate of top packages.
% % \JD{Comment on any particular places where you expect those patterns to change?}

% There could be external factors not examined in the study that significantly influence the reuse patterns of PTMs and traditional software.
% These might include community norms, regulatory changes, or shifts in technology that impact how engineers interact with these ecosystems.

% \section{Conclusions}
% In this work, we provide a quantitative perspective on the differences between the traditional software and PTM Registries.
% Prior work has examined this question qualitatively, but we are the first to quantify it and show the ways in which it does and does not hold up.
% We considered the problem from the perspective of 4 different relationships: Package-to-Package, Package-to-Reuser, Contributor-to-Package, and Reuser-to-Package.
% We report that with respect to Package-to-Reuser, and Contributor-to-Package, they are similar.
% However, with respect to Package-to-Package, and Reuser-to-Package, they are different.

% The implications of this result for researchers is that the unique attributes of PTMs provide opportunities for new metrics that better describe the effect these attributes have on reuse dynamics.
% The PTM Supply Chain also experiences 
% The implications of this result for software engineers is that the turnover of top PTMs is greater, which means that the likelihood that the same PTM is the correct choice as time goes on is lower than originally.
\section{Discussion and Implication}


\subsection{Triangulating our findings}
xxx

\subsection{Implication}
This work identified several sections where future work could further our understanding of PTM reuse.
% This work confirmed prior works suggesting that PTM selection is a more important aspect of PTM reuse than PTM synthesis.
I offer several directions for future research:


\subsubsection{Dependency Networks}
% The fundamental difference in PTM was made apparent in the difference in dependency networks among registries.
% However, there are further attributes of a PTM that were not studied that might fit a definition of a dependency (Dataset, tools used to create the model, model framework, model architecture).
% Future work that examines the relationships between models using a more complete definition of a dependency would help strengthen that comparison.
% The definition of dependency in this work resulted in a vast majority of models only having one direct dependency, there were a small subset of models that began to use multiple models together in order to achieve new functionality.
% This new function begins to resemble the synthesis found in traditional software, where many packages are depended on in order to create a new software package.
% As a result, a up-to-date study, examining the patterns of change in this domain to see if pre-models are moving towards being more synthesis based on upstream contribution then previously would be important.

In this study, the definition of dependency resulted in the majority of models having only one direct dependency.
However, a small subset of models demonstrated the use of multiple models in tandem.
This approach is beginning to mirror the synthesis found in traditional software, where numerous packages are integrated to create a new software package.
Consequently, a current study that examines the evolving patterns in this domain would be crucial to determine if PTMs are increasingly adopting a synthesis-based approach.

% \subsection{Software Licenses}
% Despite there being a much larger amount of debate around how AI models should be used, what is and isn't ethical, whether they should or should not be regulated, that has not resulted in a vastly different set of licenses for PTMs.
% Further study into the kinds of licenses that are used would help understand how Open Source PTM contributors permit reuse.

% \subsection{Contributor Patterns}
% Despite the aspects of contribution between PTMs and traditional software packages being fundamentally different, the overall larger pattern of contribution remained the same.
% Future work explaining how this similarity occurs in different contribution processes would be interesting.

\subsubsection{Package Lifespan}
The turnover of top PTMs is much greater than that of top traditional software packages.
Work that examines why this is the case would help downstream software engineers get a sense of whether or not they should allow a PTM to live past a certain period of time.

\subsubsection{Lifecycle of a Package Registry}
We acknowledge that HuggingFace may be immature as a platform for reuse.
At the time that the data was taken, HuggingFace had \TODO{X} PTMs, it now has \TODO{Y}.
As a result, it is possible that the differences in metrics is due to immaturity as a platform, rather than a special difference that sets it apart from traditional software package repositories.
We leave it for future exploration the examining of these metrics in the context of its age as a platform, and the comparison to the metrics of other traditional software packages at their age.
% \TODO{This has a basis in prior work for traditional software registries which examined }

\section{Threats to Validity} \label{sec:Threats}

\iffalse    
Every empirical research work is conducted in the real world.
Gaps between the theoretical concepts and reality, and the ways in which reality is measured, may hamper the validity of the study.
We relied heavily on prior work, and inherit the shortcomings of those works.
In addition, this paper explores novel territories, this incurring new threats as well.
\fi

% \subsection{Construct}

\paragraph{Constructs} are the operationalizations of the concepts measured in this work.
Here we highlight threats, i.e., ways in which our operationalizations may be invalid.

% The operationalization of dependency in the pre-trained model context is questionable.
There may be issues in how well the existing constructs for traditional software supply chains map onto the PTM supply chain.
The traditional concept of dependency in software packages may not directly apply to PTMs because dependencies in PTMs can manifest differently.
In traditional software, a dependency can be present in a dev environment, at build, or at runtime.
Each of these kinds of dependencies ultimately involves incorporating the functionality of a outside package into your own.
However, the nature of PTMs means that they do not have the same kinds of opportunities for other packages to incorporate into thems.
PTMs often depend on other models not for functionality but for their pretrained weights or architectures.
As a result, there is not a direct translation of dependencies from traditional software to PTMs that exists.
% The construct of licenses is also questionable in particular because the new realm of PTM's could possibly result in new kinds of licenses that aren't properly covered by the pre-existing licensed definitions.

PTMs have novel attributes compared to traditional software.
Additionally, the unique functionality that PTMs provide has also given rise to additional ethical and moral considerations compared to traditional software.
As a result, existing definitions of software licenses may not fully encompass the range of licensing arrangements used for PTMs.
It's possible that licenses which appear identical through the lens of traditional software licensing may, in fact, differ significantly when considering the impact on a PTM's reuse.
If so, these ostensibly similar licenses could have distinct implications for the reuse of PTMs, despite being classified under the same category
As a result, the differences in these licenses would not actually be expressed in the popularity of associated models.

% Dependency was intentionally chosen in order in a functional comparison.
% The purpose of dependencies in terms of their outcome and why they were studied, was examined in traditional software, and then the closest definition that would allow for the same attribute that dependency has traditional software was chosen for pre-trained models.
In order to address our concerns about dependencies, a functional comparison approach was taken.
A definition of dependencies for PTMs was chosen that mirrors the impact of dependencies in traditional software as closely as possible.
This approach sought to preserve the conceptual integrity of dependency while adapting it to the unique context of PTMs.
In the future, a definition of dependency that encompasses PTM attributes such as architecture and framework would also better represent the dependency in a PTM context.

We do not have a plan to mitigate our concerns about licenses at the moment.

% particularly the reuse patterns of Pre-Trained Models (PTMs) versus traditional software packages.

\paragraph{Internal}
% \textit{Internal} refers to the strength of association between our causes and outcomes in this work.
We highlight ways in which our results may be inaccurate and unreproducible.

% Selection of Metrics: The choice and application of metrics to compare traditional software registries with the Hugging Face ecosystem might introduce bias. If the selected metrics inherently favor the characteristics of one ecosystem over another, the results could be skewed.
% Dataset Completeness and Accuracy: The quality and completeness of the datasets used (PeaTMOSS for PTMs and Packages dataset for traditional software) could influence the study's findings. Missing data, inaccuracies, or biases in these datasets could misrepresent the actual dynamics of the ecosystems studied.
% Analysis Techniques: The methods used to analyze the datasets and interpret the results must be robust and appropriate for the data. Any limitations in the analytical techniques could lead to incorrect conclusions about the differences between traditional software and PTM registries.
The choice and application of metrics to compare traditional software registries with the Hugging Face ecosystem might introduce bias.
Many metrics that come from traditional software were developed for, and applied to a single registry in order to characterize that registry.
If the selected metrics inherently favor the characteristics of one registry over another, the results could be skewed.

Another possible issue is the completeness of the datasets used in the study (PeaTMOSS for PTMs and Packages dataset for traditional software).
These datasets aggregate self-reported metadata from the registries.
Missing data, inaccuracies, or biases could result in a misrepresentation of the studied registries.
Additionally, these datsets are ultimately snapshots of inherently volatile platforms.
As such, it is possible that these snapshots contain results that would be irreproducible with snapshots that were taken just a few months separate.

% \JD{I don't understand the relevance of the next paragraph?}
% Additionally, PTMS inherently change the dynamics compared to traditional software.
% While a traditional software registry provides the source code of a package, PTMs are typically made available through Model Zoos by providing only the model weights and definitions, which are sufficient for reuse.
% However, they do not include the code and datasets used to develop these models, potentially obscuring crucial information about the model's formation and underlying data.

To mitigate concerns regarding metric selection, we chose metrics with a proven track record across diverse software platforms, reducing the potential for bias.
Furthermore, we selected a broad spectrum of registry aspects for measurement, ensuring a comprehensive analysis of the registries in question.

% Additionally, model zoos are generally unique platforms compared to software registries.
% Where a traditional software registry provide the source code of the package, Model Zoos just provide the weights and definition of a model, just enough for it to be re-used.
% They do not provide the code and datasets that were used to create those models, which can obfuscate information about the information of the model.



% \textit{External} refers to the generalizability of our work.

\subsubsection{External} We highlight ways in which our results may not be generalizable.

% Generalizability to Other Ecosystems: The study focuses on the Hugging Face ecosystem compared to NPM and PyPi. The findings may not be generalizable to other software registries or PTM ecosystems with different characteristics or governance models.
% Evolving Nature of PTMs and Ecosystems: The rapidly evolving nature of PTMs and their ecosystems might limit the longevity of the study's findings. New trends, technologies, or practices emerging after the study's completion could alter the dynamics of PTM reuse, dependencies, and licensing.
% Influence of Unexamined Factors: There could be external factors not examined in the study that significantly influence the reuse patterns of PTMs and traditional software. These might include community norms, regulatory changes, or shifts in technology that impact how engineers interact with these ecosystems.

This study focuses on comparing the Hugging Face ecosystem to NPM and \pypi.
Existing ecosystems like NPM, \pypi, Cargo, and others have all been studied together to see if they display similar patterns of behaviors\cite{decan_empirical_2019}.
It was found that they exhibit general behaviors that are similar, but that there are differences between ecosystems in the degree of those behaviors.
% \JD{Hmm, the next sentence is a bit odd. The claimed result is that HF is not the same as npm/pypi, so the reader is wondering if we are making a bigger claim --- that HF is not the same as Crates, RubyGems, etc. The next sentence is too vague, customize it to your actual study and claimed findings}
It is important to acknowledge that our conclusions about the unique nature of HuggingFace, in contrast to NPM and \pypi, may not directly apply to other software registries such as Crates or RubyGems, which could exhibit different characteristics when evaluated using these same metrics.

The rapidly evolving nature of PTMs and their ecosystems might limit the longevity of the study's findings.
New trends, technologies, or practices emerging after the study's completion could alter the dynamics of PTM reuse, dependencies, and licensing.
It is also entirely possible that the trends shown in this study are purely due to the realtively young age of HuggingFace compared to NPM and \pypi.
HuggingFace was created in 2016, and began to explode in popularity as a platform in 2020.
For comparison, NPM was created in 2010, and \pypi was created in the early 2000s.
It may be that as HuggingFace matures as a platform, that the patterns shown here begin to resemble those of their contemporaries, especially when it comes to interpackage dependency networks and the turnover rate of top packages.
% \JD{Comment on any particular places where you expect those patterns to change?}

There could be external factors not examined in the study that significantly influence the reuse patterns of PTMs and traditional software.
These might include community norms, regulatory changes, or shifts in technology that impact how engineers interact with these ecosystems.

\section{Conclusions}
In this work, I provide a quantitative perspective on the differences between the traditional software and PTM Registries.
Prior work has examined this question qualitatively and found that PTM reuse prioritizes Selection over Synthesis, but I am the first to quantify it.
In this work, I showed that traditional software and PTM registries show differences in package evolution and reuse.
% I considered the problem from the perspective of 4 different relationships: \ptp, \ptr, \ctp and \rtp
% I show that traditional software and PTM registries show similarities in their \ptr and \ctp relationships,
% and differences in their \ptp and \rtp relationships.

% The implications of this result for researchers is that understanding the reuse patterns of downstream reuse and all the thread models and everything else all relies on PTM selection, not synthesis.
% As a result when examining engineering dynamics and other stuff, you really need to focus on the decision-making process process behind when a model is selected and when it is thrown out for a new PTM.
The implications of these findings for researchers are significant: downstream reuse patterns, package evolution, and derived information such as threat models primarily depend on PTM selection rather than synthesis.
Consequently, future work in this domain should concentrate on the processes that govern the selection of a model.

For engineers, this work emphasizes the importance of continuous evaluation of selected PTMs to ensure they remain the optimal choice for their needs.
Best practice for reuse would entail 2 things.
First, infrastructure capable of seamlessly switching betweeen PTMs.
Second, constant monitoring of updates and new models from upstream providers to determine if a new model outperforms your current model.
These two things practiced together will ensure that downstream systems are always getting the most functionality out of everything.
% For engineers, I given them the suggestion of do not go get attached to your favorite model. You should win, implementing models in your code, do this in such a way that it is possible to easily swap out the model for another likely through a layer of indirection of input to your model. I would also advise that you continuously monitor the hugging face platform for new models that are better than your current model. At whatever task you were looking for as this work shows that you are there's likely to be a higher performing model that exists shortly.

% The implications of this result for researchers is that the unique attributes of PTMs provide opportunities for new metrics that better describe the effect these attributes have on reuse dynamics.
% The implications of this result for software engineers is that the turnover of top PTMs is greater, which means that the likelihood that the same PTM is the correct choice as time goes on is lower than originally.

% \bibliography{esem}
\ifANONYMOUS
\else
\section*{Acknowledgments}

sdf
\fi

